Efficient Federated Low Rank Matrix Completion

In this work, we develop and analyze a Gradient Descent (GD) based solution, called Alternating GD and Minimization (AltGDmin), for efficiently solving the low rank matrix completion (LRMC) in a federated setting. LRMC involves recovering an $n \times q$ rank-$r$ matrix $\Xstar$ from a subset of its entries when $r \ll \min(n,q)$. Our theoretical guarantees (iteration and sample complexity bounds) imply that AltGDmin is the most communication-efficient solution in a federated setting, is one of the fastest, and has the second best sample complexity among all iterative solutions to LRMC. In addition, we also prove two important corollaries. (a) We provide a guarantee for AltGDmin for solving the noisy LRMC problem. (b) We show how our lemmas can be used to provide an improved sample complexity guarantee for AltMin, which is the fastest centralized solution.

==> altmin_coroll.tex <==
\section{Improved Guarantees for AltMin \cite{lowrank_altmin} and Smooth-AltMin}

Using the same lemmas used to prove the AltGDmin guarantee, we are also able to improve the guarantee for AltMin and Smooth-AltMin \cite{hardt2014understanding}, as long as both are initialized as given in Algorithm 1:  the initial estimate of $\U$ is clipped using row-wise clipping. We borrow this clipping idea from \cite{rpca_gd}.

\subsection{Improving the result for AltMin}

\begin{corollary}[Improved AltMin \cite{lowrank_altmin} Guarantee]
Consider the AltMin algorithm initialized using our initialization (lines 2-4) of Algorithm 1.
	%Let $\deltat := \SE_F(\U^{(t)},\U^*)$.
	Assume that Assumption \ref{incoh} holds and that, at each iteration $t$, entries of $\Xstar$ are observed independently with probability
	\begin{equation}
		p  > \frac{C  \kappa^4 \mu^2 r^2 \log q\log({1}/{\epsilon})}{n}, \label{eq:pAltMin}
	\end{equation}
	then, w.p. at least $1 - 3/n^3$, the iterates $\V^{(t)}$ of AltMinComplete \cite{lowrank_altmin} satisfy $\SE_F(\V^{(t+1)},\V^*)  \leq \frac{1}{2} \SE_F(\U^{(t)},\U^*).$\label{thm:AltMinCmplt}
\label{altmin_thm}
\end{corollary}

Comparing \eqref{eq:pAltMin}  to Theorem 2.5 of \cite{lowrank_altmin}, we observe that the sample complexity for AltMinComplete has reduced in $r$ from $r^{4.5} \log r$ to $r^2$, and from $\log(\lV \X^* \rV_F/\eps)$ to $\log(1/\eps)$. The proof of this result is follows from Lemmas \ref{lem:init}, \ref{lem:BerrLmma} and \ref{lem:Berr_implic}. We provide the proof in Sec. \ref{altmin_thm_proof}. %along with using the algebra from the original AltMin paper.


	\subsection{Proof of Corollary \ref{altmin_thm}: move to Appendix after fixing it - keep proof short}\label{altmin_thm_proof}

	%\begin{proof}[Proof of Theorem \ref{altmin_thm}]
	%The proof is an easy consequence of Lemma \ref{lem:BerrLmma} and Lemma \ref{init}.
	%Recall $\B^\intercal \qreq \V\R$, and
	In section 4.2 of \cite{lowrank_altmin}, it is shown that the least-squares updates for $\U \in \mathbb{R}^{n \times r}$ and $\B \in \mathbb{R}^{r \times q}$ are equivalent to the following QR-based updates:
	\begin{align}
		 \B^{(t)} &= \argmin_{ \B} \lV \Y - \U^{(t)}  \B \rV_F^2, \,\,\,   \B^{(t)\intercal} \qreq \V^{(t)}\R_{\B} \label{eq:BLS_Updt}\\
		\widetilde \U^{(t+1)} &=  \argmin_{\widetilde \U} \lV \Y^\intercal - \V^{(t)} \widetilde \U \rV_F^2, \,\,\, \widetilde \U^{(t+1)^\intercal} \qreq \U^{(t+1)}\R_\U. \label{eq:ULS_Updt}
	\end{align}
	\subsubsection{$\mathbf{B}$-update \eqref{eq:BLS_Updt}\,/\,$\SE_F(\mathbf V^{(t)},\mathbf V^*)$ Bound}
	Note that the $\B$-update in \eqref{eq:BLS_Updt} is exactly the same as the $\B$-update for AltGDMin. Therefore, we use Lemma \ref{lem:BerrLmma} to bound $\SE_F(\V^{(t)},\V^*)$. Let $\P \coloneq \mathbf{I} - \V^*\V^{*\intercal}$. Then,
	\begin{align} \SE_F(\V^{(t)},\V^*)  &= \lV  \P \V^{(t)} \rV_F = \lV  \P \B^{\intercal} \R_{B}^{-1} \rV_F \leq \lV \P \B^\intercal  \rV_F \lV \R_{B}^{-1}\rV \leq {\lV (\B-\G)^\intercal \rV_F}/{\sigma_{\min}(\B)}, \label{eq:SEF_AltMin}
	\end{align}
	where $\P\B^\intercal = \P(\G^\intercal + (\B-\G)^\intercal) = \P(\B - \G)^\intercal$, because $\G^\intercal = \X^{*\intercal}\U^\intercal$  and the column-span of $\X^{*\intercal}$ is orthogonal to the span of $\P$.
By Lemma \ref{lem:BerrLmma}, (with $\eps = 1/(8 \kappa \sqrt{r}))$, $\lV  \B - \G \rV_F \leq \sigmin \deltatold/4$. By Lemma \ref{lem:Berr_implic},  assuming $\deltatold \leq 1/(4\kappa)$, $\sigma_{\min}(\B) \geq \sigmin/2$.  Substituting these bounds in \eqref{eq:SEF_AltMin} and recalling that $\deltatold \coloneq \SE_F(\U^{(t)},\U^*)$, w.p. greater than $1 - \exp(\log q - pn/(r^2 \mu^2\kappa^4))$,
	\begin{equation}
		\SE_F(\V^{(t)},\V^*) \leq  \frac{1}{2} \SE_F(\U^{(t)},\U^*). \label{eq:altMinVBnd}
	\end{equation}
	%Since, both $\U$ and $\B$ are updated by the least-squares solution, Lemma \ref{lem:BIncohLmma} applies to give $\mu$-incoherence for the rows of $\U$ and columns of $\B$.
	\subsubsection{Incoherence of $\mathbf{V}^{(t)}$} Recall that $\widetilde \B^\intercal \qreq \V\R$. Then, the $k$-th row, $\lV \v^k \rV_2  \leq {\lV \b_k\rV_2}/{\sigmin(\B)} \leq C \kappa \mu \sqrt{r/q}$, where the last inequality follows from Lemmas \ref{lem:Berr_implic} and  \ref{lem:BIncohLmma}. Thus, $\V$ is $\kappa \mu$-incoherent.
	\subsubsection{$\mathbf{U}$-Update \eqref{eq:ULS_Updt}\,/\,$\SE_F(\mathbf{U^{(t+1)}},\mathbf{U}^*)$ Bound} Given that the sensing matrix $\V^{(t)}$ in \eqref{eq:ULS_Updt} is i) orthronormal, ii) $\SE_F(\V^{(t)},\Vstar) \leq \frac{1}{2} \SE_F(\U^{(t)},\U^*) \leq \frac{1}{2} \delta$ and, iii) $\kappa \mu$-incoherent, we can bound $\lV \widetilde \U - \G_V \rV_F$, where $\G_V = \V^{(t)\intercal}\X^{*\intercal}$, similarly to Lemma \ref{lem:BerrLmma}. Therefore, with probability greater than  $1 - \exp(\log n - pq/(r^2 \mu^2\kappa^4))$,
		\begin{equation}
		\SE_F(\U^{(t+1)},\U^*) \leq  \frac{1}{2} \SE_F(\V^{(t)},\U^*). \label{eq:altMinUBnd}
	\end{equation}
	\subsubsection{Incoherence of $\mathbf{U}^{(t+1)}$} Lemma \ref{lem:BIncohLmma} applies to give row-incoherence $\lV \tilde \u^j \rV_2 \leq \sigmax \mu \sqrt{r/n}$ and $\kappa \mu$-row incoherence follows similarly as $\kappa \mu$-column incoherence for $\V$ in 2) above, that is, by lower bounding $\sigma_{\min}(\tilde \U)$.
	
	Combining \eqref{eq:altMinVBnd} and $\eqref{eq:altMinUBnd}$, we have $\SE_F(\U^{(t+1)},\U^*) \leq \SE_F(\U^{(t)},\U^*)/4 $. For initialization we use the few lines of our Algorithm 1 and Lemma \ref{lem:init}.  %By Lemma \ref{lem:init}, $\U$ has incoherence $\mu_{\u} \leq \kappa \mu$.
Consequently, AltMinComplete  \cite{lowrank_altmin} initialized as given in the first few lines of our Algorithm 1  needs $T =\log(1/\eps)$ iterations for $\SE_F(\U^{(t)},\U^*) \leq \eps $.
	%\subsubsection{Lemma \ref{lem:BerrLmma} bound for $\mathbf{U}$ least-squares update}


\subsection{Improved Guarantee for Smooth AltMin \cite{hardt2014understanding}}
We will reduce the overall sample complexity by decreasing $p_{init}$ to $O(r^2)$ below.  Formally,
%\begin{corollary}
%	Given a size of $O(pn^2)$ drawn from an unknown $n \times n$ matrix $\Xstar$ of rank-$r$ by including each entry with probability $p$, SAltLS \cite{hardt2014understanding} outputs with high probability $\U$, $\B$ such that $\lV (\I - \U^*\U^{*\intercal})\U \rV \leq \eps$ and $\lV X - \U\B \rV_F \leq \eps \lV \Xstar \rV_F$ provided that
%	\begin{equation}
%		pn \geq r^2 (r + \log(n/\eps)) \mu \kappa^2.
%	\end{equation}
%\end{corollary}
\begin{corollary} Let $r, \eps > 0$. Let $\Xstar$ be a symmetric $n \times n$ matrix. Then, for $T = O(\log(n/\eps))$,  the output of SAltLS satisfies $\SE_F (\U,\U^*) \leq \eps$ with probability $9/10$, provided that sampling probability $p \geq p_{init} + p_{LS}$, where
\begin{equation}
	p_{\mathrm{init}} \geq C{ \kappa^2 r^2 \mu  \log n}/{n },
	%p_{init} \geq C{ \kappa^2 r^2 \mu  \log q}/{(n  )}%,
	\quad  p_{\mathrm{LS}}  \geq C{ \mu^2\kappa^2 r^2 \log(n/\eps)\log^2 n}/{n}.
	\label{eq:HardtNew}
\end{equation}
\end{corollary}

This is a direct corollary of Theorem 6.1 of \cite{hardt2014understanding} combined with our initialization lemma, Lemma \ref{lem:init}.

%\begin{proof}
%Compared to equation (9) in Theorem 7.1 of \cite{hardt2014understanding} (the initialization guarantee therein), which requires $O(r^3)$ sample complexity,  $p_{\textrm{init}}$ in \eqref{eq:HardtNew} needs $p \geq   C{r^2 \ \kappa^2 \mu \log n}/{ n}$ to output a $\mu$-incoherent $\U$. Consequently, by invoking Lemma \ref{lem:init}, instead of Theorem 7.1 of \cite{hardt2014understanding}  we have reduced $p_{init}$ in \eqref{eq:HardtNew} from $r^3$ dependence to $r^2$. We only modify the initialization of SAltLS algorithm so that the $p_{\mathrm{LS}}$ in \eqref{eq:HardtNew} does not change.
%
%%	From section 6 of \cite{hardt2014understanding}, the sampling complexity of SmoothAltMin (SAltLS), for the noise less case,  is the sum of the following two quantities:%
%%	\begin{equation}
%%		p_{init} = {  r^3  \kappa^2  \mu\log q}/{q}, \quad p_{LS} = { \mu^2\kappa^2 r^2 \log(q/\eps)\log^2 q}/{q}. \label{eq:HardtInit}
%%	\end{equation}
%\end{proof}


%First, we rewrite the initialization guarantee (Theorem 7.1 from \cite{hardt2014understanding}), assuming zero noise, in our notation.
%\begin{corollary} Let $\Xstar$  be a symmetric $q \times q$, $\mu$-incoherent matrix rank $r$ matrix. Assume that each entry is included in $\Omega$ independently with probability
%\begin{equation}
%p \geq \frac{C r^3\kappa^2\mu\log q}{q} \label{eq:pHardt}
%\end{equation}
%for a sufficiently large constant $C > 0$. Then, the algorithm INITIALIZE \cite{hardt2014understanding} returns an orhtonormal matrix $\U^{(0)}$ such that with probability $9/10$,  $\SE_F(\U^{(0)},\U^*) \leq 1/4$ and $\mu(\U^{(0)}) \leq 32 \mu \log q$.	\label{thm:SAltMinInit}
%\end{corollary}


%?? edit this to also add Final Result for Smooth AltMin - just borrow their theorem of their paper and combine to give ONE FINAL result.


%\subsection{Proof of Corollary \ref{altmin_thm}: move to Appendix after fixing it - keep proof short}\label{altmin_thm_proof}
%
%%\begin{proof}[Proof of Theorem \ref{altmin_thm}]
%The proof is an easy consequence of Lemma \ref{lem:BerrLmma} and Lemma \ref{init}.
%
%Let $\B^\intercal \qreq \V\R$, and let $\P \coloneq \mathbf{I} - \V^*\V^{*\intercal}$. Then,
%\begin{align} \SE_F(\V,\V^*)  &= \lV  \P \V \rV_F = \lV  \P \B^\intercal \R^{-1} \rV_F \leq \lV \P \B^\intercal  \rV_F \lV \R^{-1}\rV \notag\\
%&\leq {\lV (\B-\G)^\intercal \rV_F}/{\sigma_{\min}(\B)}, \label{eq:SEF_AltMin}
%\end{align}
%where we have used that  $\P\B^\intercal = \P(\G^\intercal + (\B-\G)^\intercal) = \P(\B - \G)^\intercal$, because $\G^\intercal = \X^{*\intercal}\U^\intercal$  and the column-span of $\X^{*\intercal}$ is orthogonal to the span of $\P$. By Lemma \ref{lem:BerrLmma}, (with $\eps = 1/(8 \kappa \sqrt{r}))$, $\lV  \B - \G \rV_F \leq \sigmin \deltat/4$. By Lemma \ref{lem:Berr_implic},  assuming $\deltat \leq 1/(4\kappa)$, $\sigma_{\min}(\B) \geq \sigmin/2$.  Substituting these bounds in \eqref{eq:SEF_AltMin} and recalling that $\deltat \coloneq \SE_F(\U^{(t)},\U^*)$, w.p. greater than $1 - \exp(\log q - pn/(r^2\kappa^4\mu^4))$,
%\begin{equation}
%	\SE_F(\V,\V^*) \leq  \frac{1}{2} \SE_F(\U^{(t)},\U^*).
%\end{equation}
%Since, both $\U$ and $\B$ are updated by the least-squares solution, Lemma \ref{lem:BIncohLmma} applies to give $\mu$-incoherence for the rows of $\U$ and columns of $\B$.
%?? fix this - show incoh of vk. say we need $T = \log(1/\eps)$
%%\end{proof}



==> improved_altmin_coroll.tex <==
\section{Improved Guarantees for AltMin \cite{lowrank_altmin} and Smooth-AltMin} \label{altmincorolls}

Using the same lemmas used to prove the AltGDmin guarantee, we are also able to improve the guarantee for AltMin and Smooth-AltMin \cite{hardt2014understanding}, as long as both are initialized as given in Algorithm 1:  the initial estimate of $\U$ is clipped using row-wise clipping. We borrow this clipping idea from \cite{rpca_gd}.

\subsection{Improving the result for AltMin}

\begin{corollary}[Improved AltMin \cite{lowrank_altmin} Guarantee]
Consider the AltMin algorithm initialized using our initialization (lines 2-4) of Algorithm 1.
	%Let $\deltat := \SE_F(\U^{(t)},\U^*)$.
	Assume that Assumption \ref{incoh} holds and that, at each iteration $t$, entries of $\Xstar$ are observed independently with probability
	\begin{equation}
		p  > \frac{C  \kappa^4 \mu^2 r^2 \log q\log({1}/{\epsilon})}{n}, \label{eq:pAltMin}
	\end{equation}
	then, w.p. at least $1 - 3/n^3$, the iterates $\V^{(t)}$ of AltMinComplete \cite{lowrank_altmin} satisfy $\SE_F(\V^{(t+1)},\V^*)  \leq \frac{1}{2} \SE_F(\U^{(t)},\U^*).$\label{thm:AltMinCmplt}
\label{altmin_thm}
\end{corollary}

We prove this in Appendix \ref{altmin_thm_proof}.
Comparing \eqref{eq:pAltMin}  to Theorem 2.5 of \cite{lowrank_altmin}, we observe that the sample complexity for AltMinComplete has reduced in $r$ from $r^{4.5} \log r$ to $r^2$, and from $\log(\lV \X^* \rV_F/\eps)$ to $\log(1/\eps)$. The proof of this result  follows from Lemmas \ref{lem:init}, \ref{lem:BerrLmma} and \ref{lem:Berr_implic}. We provide the proof in Sec. \ref{altmin_thm_proof}. %along with using the algebra from the original AltMin paper.


\subsection{Improved Guarantee for Smooth AltMin \cite{hardt2014understanding}}
We will reduce the overall sample complexity by decreasing $p_{init}$ to $O(r^2)$ below.  Formally,
%\begin{corollary}
%	Given a size of $O(pn^2)$ drawn from an unknown $n \times n$ matrix $\Xstar$ of rank-$r$ by including each entry with probability $p$, SAltLS \cite{hardt2014understanding} outputs with high probability $\U$, $\B$ such that $\lV (\I - \U^*\U^{*\intercal})\U \rV \leq \eps$ and $\lV X - \U\B \rV_F \leq \eps \lV \Xstar \rV_F$ provided that
%	\begin{equation}
%		pn \geq r^2 (r + \log(n/\eps)) \mu \kappa^2.
%	\end{equation}
%\end{corollary}
\begin{corollary} Let $r, \eps > 0$. Let $\Xstar$ be a symmetric $n \times n$ matrix. Then, for $T = O(\log(n/\eps))$,  the output of SAltLS satisfies $\SE_F (\U,\U^*) \leq \eps$ with probability $9/10$, provided that sampling probability $p \geq p_{init} + p_{LS}$, where
\begin{equation}
	p_{\mathrm{init}} \geq C{ \kappa^2 r^2 \mu  \log n}/{n },
	%p_{init} \geq C{ \kappa^2 r^2 \mu  \log q}/{(n  )}%,
	\quad  p_{\mathrm{LS}}  \geq C{ \mu^2\kappa^2 r^2 \log(n/\eps)\log^2 n}/{n}.
	\label{eq:HardtNew}
\end{equation}
\end{corollary}
This is a direct corollary of Theorem 6.1 of \cite{hardt2014understanding} combined with our initialization lemma, Lemma \ref{lem:init}.

%\begin{proof}
%Compared to equation (9) in Theorem 7.1 of \cite{hardt2014understanding} (the initialization guarantee therein), which requires $O(r^3)$ sample complexity,  $p_{\textrm{init}}$ in \eqref{eq:HardtNew} needs $p \geq   C{r^2 \ \kappa^2 \mu \log n}/{ n}$ to output a $\mu$-incoherent $\U$. Consequently, by invoking Lemma \ref{lem:init}, instead of Theorem 7.1 of \cite{hardt2014understanding}  we have reduced $p_{init}$ in \eqref{eq:HardtNew} from $r^3$ dependence to $r^2$. We only modify the initialization of SAltLS algorithm so that the $p_{\mathrm{LS}}$ in \eqref{eq:HardtNew} does not change.
%
%%	From section 6 of \cite{hardt2014understanding}, the sampling complexity of SmoothAltMin (SAltLS), for the noise less case,  is the sum of the following two quantities:%
%%	\begin{equation}
%%		p_{init} = {  r^3  \kappa^2  \mu\log q}/{q}, \quad p_{LS} = { \mu^2\kappa^2 r^2 \log(q/\eps)\log^2 q}/{q}. \label{eq:HardtInit}
%%	\end{equation}
%\end{proof}


%First, we rewrite the initialization guarantee (Theorem 7.1 from \cite{hardt2014understanding}), assuming zero noise, in our notation.
%\begin{corollary} Let $\Xstar$  be a symmetric $q \times q$, $\mu$-incoherent matrix rank $r$ matrix. Assume that each entry is included in $\Omega$ independently with probability
%\begin{equation}
%p \geq \frac{C r^3\kappa^2\mu\log q}{q} \label{eq:pHardt}
%\end{equation}
%for a sufficiently large constant $C > 0$. Then, the algorithm INITIALIZE \cite{hardt2014understanding} returns an orhtonormal matrix $\U^{(0)}$ such that with probability $9/10$,  $\SE_F(\U^{(0)},\U^*) \leq 1/4$ and $\mu(\U^{(0)}) \leq 32 \mu \log q$.	\label{thm:SAltMinInit}
%\end{corollary}


%?? edit this to also add Final Result for Smooth AltMin - just borrow their theorem of their paper and combine to give ONE FINAL result.


%\subsection{Proof of Corollary \ref{altmin_thm}: move to Appendix after fixing it - keep proof short}\label{altmin_thm_proof}
%
%%\begin{proof}[Proof of Theorem \ref{altmin_thm}]
%The proof is an easy consequence of Lemma \ref{lem:BerrLmma} and Lemma \ref{init}.
%
%Let $\B^\intercal \qreq \V\R$, and let $\P \coloneq \mathbf{I} - \V^*\V^{*\intercal}$. Then,
%\begin{align} \SE_F(\V,\V^*)  &= \lV  \P \V \rV_F = \lV  \P \B^\intercal \R^{-1} \rV_F \leq \lV \P \B^\intercal  \rV_F \lV \R^{-1}\rV \notag\\
%&\leq {\lV (\B-\G)^\intercal \rV_F}/{\sigma_{\min}(\B)}, \label{eq:SEF_AltMin}
%\end{align}
%where we have used that  $\P\B^\intercal = \P(\G^\intercal + (\B-\G)^\intercal) = \P(\B - \G)^\intercal$, because $\G^\intercal = \X^{*\intercal}\U^\intercal$  and the column-span of $\X^{*\intercal}$ is orthogonal to the span of $\P$. By Lemma \ref{lem:BerrLmma}, (with $\eps = 1/(8 \kappa \sqrt{r}))$, $\lV  \B - \G \rV_F \leq \sigmin \deltat/4$. By Lemma \ref{lem:Berr_implic},  assuming $\deltat \leq 1/(4\kappa)$, $\sigma_{\min}(\B) \geq \sigmin/2$.  Substituting these bounds in \eqref{eq:SEF_AltMin} and recalling that $\deltat \coloneq \SE_F(\U^{(t)},\U^*)$, w.p. greater than $1 - \exp(\log q - pn/(r^2\kappa^4\mu^4))$,
%\begin{equation}
%	\SE_F(\V,\V^*) \leq  \frac{1}{2} \SE_F(\U^{(t)},\U^*).
%\end{equation}
%Since, both $\U$ and $\B$ are updated by the least-squares solution, Lemma \ref{lem:BIncohLmma} applies to give $\mu$-incoherence for the rows of $\U$ and columns of $\B$.
%?? fix this - show incoh of vk. say we need $T = \log(1/\eps)$
%%\end{proof}



==> improved_lrmc_altgdmin_noisy.tex <==

\section{Proof of the noisy case}

We observe
\[
\Y = \Xstar_\Omega + \W_\Omega
\]
First assume deterministic $\w_\jk$s and assume $\w_\jk^2 \le  \sigma_w^2$
%Assume $w_\jk$ are i.i.d. zero mean Gaussian with variance $\sigma_w^2$.

\subsection{Initialization}
Using spectral-methods-paper Lemma 3.21 and Wedin's sin theta theorem,
\[
\SE_F(\U_00, \Ustar) \le 2 \frac{||\Y - \Xstar||_F}{\sigmin - 0} \le  2\frac{||\Xstar_\Omega- \Xstar||_F + ||\W_\Omega ||_F}{\sigmin - 0}
\]

First term - use Lemma 3.21. Second term -
\[
\E[||\W_\Omega ||_F^2] \le \E[|\Omega|] \sigma_w^2  = (nq p ) \sigma_w^2
\]
Deviation -- bound $\sum_\jk (\zeta_\jk^2 - p) \w_\jk^2$ - use scalar Bernstein to show that this is $\le \eps (nq p ) \sigma_w^2$ whp. So then
$||\W_\Omega||_F \le C \sqrt{nqp} \sigma_w$ whp.

We need $ C \sqrt{nqp} \sigma_w \le \delta_0/5$ or $\sigma_w \le c \delta_0 / \sqrt{nq p} $.

\subsection{Iterations - B-G}
1. bound $B-G$ --
2. bound gradient

$B-G$ bound:
\[
\b_k - \g_k = Term_k + TermNoise_k, \ TermNoise_k = \F_k^{-1} \U_k^\top \w_k
\]


\[
||\E[\U_k' w_k]|| = p ||\sum_j \u_j w_\jk||= p \sqrt{||\sum_j \u_j w_\jk||^2} \le p \sqrt{ \sum_j ||\u_j||^2 w_\jk^2} \le p \sigma_w \sqrt{r}
% \le \sum_j  ||\u_j|| \cdot |w_\jk| \le \mu_u \sqrt{r/n}
\]
since $||\U||_F^2 = r$.
Can show that whp $||\U_k' w_k||^2 \le C\sigma_w^2 (p r )$ and that $||TermNoise||_F^2 \le C (q p r ) \sigma_w^2$

Proceeding as before,
\[
||TermNoise||^2 = || \sum_k (\U_k^\top \w_k) \e_k^\top || = ||\sum_\jk \zeta_\jk \w_\jk  \u_j \e_k^\top ||
\]
$\E[.] = p  \sum_\jk \w_\jk \u_j \e_k^\top $

if consider Gaussian noise, then $\E[.] = 0$. try using:
- first condition $\w_\jk$s and use matrix Bern. then uncondition . when applying matrix Bern $x_\jk  - \xstar_\jk$ is getting replaced by $\w_\jk$
so 
\\
$L = \max_\jk |\w_\jk| . \mu \sqrt{r/q} \sigmax$
and
$\sigma^2 = p \mu^2 (r/q) . ||\W||_F^2 \le p \mu^2 (r/q) . (nq) \max_\jk |\w_\jk|^2 = np \mu^2 r  \max_\jk |\w_\jk|^2 $
 


\subsection{Gradient term}
\[
GradNoise= \sum_\jk \zeta_\jk \w_\jk \e_j \b_k'
\]


==> improved_lrmc_noisy_altmincoroll_proofs.tex <==

%\newcommand{\w}{\bm{w}}

\section{Guarantee for Noisy LRMC}
Consider the noisy LRMC problem defined as follows. We observe
\[
\Y := \Xstar_\Omega + \W_\Omega
\]
and do not make any assumption on the noise $\W$ (deterministic $\W$).  Unlike the standard Gaussian assumption, this assumption is weaker: it allows the noise entries to be anything, all entries could be positive too for example.

We can show the following by borrowing the overall proof approach for modifying a noise-free case proof from \cite{twf} and \cite{lrpr_best} (the latter used a similar approach for analyzing the AltMin algorithm for LR phase retrieval).

%Assume $w_\jk$ are i.i.d. zero mean Gaussian with variance $\sigma_w^2$.

\begin{corollary}
??
Let
\[
\eps_noise := \max(\frac{\max_k \|\w_k\|}{\max_k \|\xstar_k\|}, \frac{\max_j \|\w^j\|}{\max_j \|\xstar{}^j\|}
\]
In the setting of Theorem \ref{thrm}, if
$
\eps_{noise} \le  \frac{c}{\kappa^3}, ??
%\|\W\|_F \le c \frac{1}{\kappa^2} \sigmin
$
then, by setting $T = C \kappa^2 \log(1/\eps_{noise})$, we can guarantee that
\[
\SE(\U,\Ustar) \le \eps_{noise} \ \text{ and } \  \|\X- \Xstar\|_F \le \eps_{noise} \sigmax = C \|\W\|_F
\]
In general, for any $\eps$, by setting $T = C \kappa^2 \log(1/\eps)$, we can ensure that
$\SE(\U,\Ustar) \le \max(\eps,\eps_{noise})$ and $\|\X- \Xstar\|_F \le \max(\eps \|\Xstar\|, C \|\W\|_F)$.
\label{cor_noisy}
\end{corollary}

\begin{proof}
The proof is a natural extension of our proof for the noise-free case.
Corollary \ref{cor_noisy} extends our proof to the noisy case using the following simple ideas. First we assume that the noise level is small enough so that accurate initialization is possible; this requires noise level to be of order $c \delta_0 \sigmin$ for our required value of $\delta_0 = c/\kappa^2$. Next, at each iteration, in order to be able to guarantee error decay similar to the noise-free case, we need the noise level to be such that (i) the error in recovering $\Bstar$ is of the same order as in the noise-free case; and (ii) the same is true for the gradient norm. Both of these are ensured if the noise Frobenius norm $\|\W\|_F$ is below $c \delta_t \sigmax$ at iteration $t$. Said another way, the error will decay as long as $\delta_t \ge \eps_{noise} = C \|\W\|_F/\sigmax$. The proof is in Appendix \ref{proof_noisy}
\end{proof}


\section{Proof of the noisy case} \label{proof_noisy}

\newcommand{\bw}{\|\W\|_{\max}}

We observe
\[
\Y := \Xstar_\Omega + \W_\Omega
\]
and we assume the noise is deterministic. Unlike the standard Gaussian assumption, this assumption is a weaker one: it allows the noise entries to be anything, all entries could be positive too for example.
%Assume deterministic $\w_\jk$s and use $\bw$ to denote its maximum magnitude entry.
%Assume $w_\jk$ are i.i.d. zero mean Gaussian with variance $\sigma_w^2$.

\subsection{Iterations}
Assume $\SE_F(\U, \Ustar) \le \delta_0$ as before. Our goal is to find conditions under which all the bounds on the terms in the $\SE_F(\U^+, \Ustar)$ remain the same. This ensures that the algebra of Sec. \ref{proof_theorem} applies.

With the noise, the following will change for the terms that need to be bounded.
\bi
\item $\|\B - \G\|_F \le \|\F^{-1}\|  (\|\D\|_F  + NoiseTerm_B) $ where
\[
NoiseTerm_B = \sum_k \U_k^\intercal \w_k \e_k^\intercal
\]
\bi
\item  Since $\E[NoiseTerm_B] = p \sum_k  (\U^\intercal \w_k) \e_k^\intercal = p \U^\intercal \W$, we have $\|\E[NoiseTerm_B]\|_F = p \|\U^\intercal \W\|_F  = p\|\W\|_F $
\item Proceeding as in the noise-free case (use matrix Bernstein), if we assume
\begin{align}
\max_k \|\w_k\| \le \eps_noise \max_k  ||\xstar_k|| , \   \max_j \|\w^j\| \le \eps_noise \max_j  ||\xstar^j||
\label{assuw}
\end{align}
then, we can show that, whp,
\[
\|NoiseTerm_B \| \le  p c  \deltatold \sigmax
\]


\item From earlier, $\|\D\|_F \le p c  \deltatold \sigmax $
\item Thus if \eqref{assuw} holds,
%\[
%\|\W\|_F  \le  c \deltat \sigmax
%\]
then the $\|\B - \G\|_F$ bound remains the same as earlier.
\ei

%\item If same $\|\B - \G\|_F$ bound, then $\gradU] = \E[OldTerm] + \E[

\item $\gradU = OldTerm + NoiseTerm_U$ where
\[
NoiseTerm_U = \sum_\jk \zeta_\jk \w_\jk \e_j \b_k^\intercal
\]
If  the $\|\B - \G\|_F$ bound remains the same as earlier, then
\bi
\item Bound on $\|\E[OldTerm]\|$ and on the deviation from mean both remain the same. From earlier, we have $\|\E[OldTerm]\|_F \le 1.1 p \deltatold \sigmax^2 $ and $\|OldTerm - \E[OldTerm] \| \le c p   \deltatold \sigmax^2$.

\item We have $\E[NoiseTerm_U] = p \sum_\jk  \w_\jk \e_j \b_k^\intercal =p \sum_k (\sum_j  \w_\jk \e_j) \b_k^\intercal = p \sum_k \w_k \b_k^\intercal = p \W \B^\intercal$ and thus $\|.\|_F \le 1.1 p \|\W\|_F \sigmax$.
  Proceeding as in noise-free case  (use matrix Bernstein), whp,
%$\|NoiseTerm_U - \E[NoiseTerm_U] \|_F \le c p \|\W\|_F \sigmax $. Thus, whp,
%\[
%\|NoiseTerm_U\|_F \le 1.1 p \|\W\|_F \sigmax + c p \|\W\|_F \sigmax \le 1.5 p \|\W\|_F \sigmax
%\]
\[
\|NoiseTerm_U\|_F \le c p   \deltatold \sigmax^2.
\]

%\item We have
%\[
%\|\E[\gradU]\|_F \le \|\E[OldTerm]\|_F  + 1.1 p \|\W\|_F \sigmax
%\]


%\item Thus,
%\[
%\|\gradU - \E[\gradU] \|_F  \le \|OldTerm - \E[OldTerm]\|_F  + c p \|\W\|_F \sigmax
%\]

\ei

\item When doing the algebra for bounding $\SE_F(\U,\Ustar)$, ?? fix the rest if above is correcgt
\bi
\item the numerator second term is $\|OldTerm - \E[OldTerm]\|_F + \|NoiseTerm_U\|_F$ instead of just $\|OldTerm - \E[OldTerm]\|_F$.
\item the denominator second term is $\|OldTerm\| + \|NoiseTerm_U\|$.
\item for the algebra to go through, we need numerator term bounded by $c p   \deltatold \sigmax^2$ with a $c < 1$. Thus this is what controls the noise requirement, i.e., we need
$\|NoiseTerm_U\|_F \le c p   \deltatold \sigmax^2$.

\item Thus, if
\[
\|\W\|_F   \le   c \deltatold \sigmax
\]
then $\SE_F$ algebra remains the same too.
%\[
%1.5 p \|\W\|_F \sigmax \le   c p \deltatold \sigmax^2  \ \text{ or }  \|\W\|_F   \le   c  \deltatold \sigmax
%\]
\ei

\item Thus, if $\|\W\|_F   \le   c \deltatold \sigmax $, then $\deltat$ decays as before. In other words, error decays exponentially until it reaches the noise level,
\[
\eps_{noise} = C \|\W\|_F / \sigmax.
\]

\item In summary, by setting $T = C \kappa^2 \log(1/\eps_{noise})$, we can guarantee that
\[
\SE(\U,\Ustar) \le \eps_{noise}, \|\X- \Xstar\|_F \le \eps_{noise} \sigmax = C \|\W\|_F
\]
In general, for any $\eps$, by setting $T = C \kappa^2 \log(1/\eps)$, we can ensure
$\SE(\U,\Ustar) \le \max(\eps,\eps_{noise})$ and $\|\X- \Xstar\|_F \le \max(\eps \|\Xstar\|, C \|\W\|_F)$.

\ei

As in all previous under-determined problems, one can only guarantee recovery up to $C \|\W\|_F$ error level. %We cannot increase the number of samples to g
Only in oversampled settings (e.g. standard Least Squares), we can get recovery error less than noise norm.


\subsection{Initialization}
Using spectral-methods-paper Lemma 3.21 and Wedin's sin theta theorem (Frob norm version),
\[
\SE_F(\U^{(00)}, \Ustar) \le C \frac{\|\Y - \Xstar\|_F}{\sigmin - 0}
\le  C \frac{\|\Xstar_\Omega- \Xstar\|_F + \|\W_\Omega \|_F}{p \sigmin - 0}
%\le  C \frac{p \sqrt{\frac{\mu r^2 \log n}{p}} \sigmax  + \|\W_\Omega \|_F}{\sigmin - 0}
\le C  \sqrt{\frac{\kappa^2 \mu r^2 \log n}{p}}   + (\|\W_\Omega \|_F / p \sigmin)
\]
The first term is bounded by $\delta_0$ under the assumption on $p$ given in the noise-free case.
For the noise term, we again show that $\|\W_\Omega\|_F \le 1.1 p \|\W\|_F$.
Thus, if
\[
\|\W\|_F \le \delta_0 \sigmin
\]
then initialization guarantee does not change.

\subsection{Final conclusion}
We need $\|\W\|_F \le c \delta_0 \sigmin $ for $\delta_0 = c/\kappa^2$. Thus,
\begin{corollary}
Let $\eps_{noise} = C \|\W\|_F / \sigmax.$
If
\[
\|\W\|_F \le c \frac{1}{\kappa^2} \sigmin
\]
then, by setting $T = C \kappa^2 \log(1/\eps_{noise})$, we can guarantee that
\[
\SE(\U,\Ustar) \le \eps_{noise}, \  \|\X- \Xstar\|_F \le \eps_{noise} \sigmax = C \|\W\|_F
\]
In general, for any $\eps$, by setting $T = C \kappa^2 \log(1/\eps)$, we can ensure
$\SE(\U,\Ustar) \le \max(\eps,\eps_{noise})$ and $\|\X- \Xstar\|_F \le \max(\eps \|\Xstar\|, C \|\W\|_F)$.
\end{corollary}




%\section{Do}
%Contribution: Treating $\kappa,\mu$ as numerical constants we argue that AltGDmin and FactGD both have the same and lowest total time cost, AltGDmin also has the lowest communication cost. AltGDmin has the second smallest sample complexity; it is worse than that of FactGD by a factor of $\log(1/\eps)$.
 %Table: sample, iter, time per iter, comm per iter. with kappa mu.



%First term - use Lemma 3.21. Second term -
%\[
%\E[\|\W_\Omega \|_F^2] \le \E[|\Omega|] \sigma_w^2  = (nq p ) \sigma_w^2
%\]
%Deviation -- bound $\sum_\jk (\zeta_\jk^2 - p) \w_\jk^2$ - use scalar Bernstein to show that this is $\le \eps (nq p ) \sigma_w^2$ whp. So then
%$\|\W_\Omega\|_F \le C \sqrt{nqp} \sigma_w$ whp.
%
%We need $ C \sqrt{nqp} \sigma_w \le \delta_0/5$ or $\sigma_w \le c \delta_0 / \sqrt{nq p} $.
%




%\clearpage \section{delete}
%
%
%$B-G$ bound:
%\[
%\b_k - \g_k = Term_k + TermNoise_k, \ TermNoise_k = \F_k^{-1} \U_k^\intercal \w_k
%\]
%
%
%\[
%\|\E[\U_k' w_k]\| = p \|\sum_j \u_j w_\jk\|= p \sqrt{\|\sum_j \u_j w_\jk\|^2} \le p \sqrt{ \sum_j \|\u_j\|^2 w_\jk^2} \le p \sigma_w \sqrt{r}
%% \le \sum_j  \|\u_j\| \cdot |w_\jk| \le \mu_u \sqrt{r/n}
%\]
%since $\|\U\|_F^2 = r$.
%Can show that whp $\|\U_k' w_k\|^2 \le C\sigma_w^2 (p r )$ and that $\|TermNoise\|_F^2 \le C (q p r ) \sigma_w^2$
%
%Proceeding as before,
%\[
%\|TermNoise\|^2 = \| \sum_k (\U_k^\intercal \w_k) \e_k^\intercal \| = \|\sum_\jk \zeta_\jk \w_\jk  \u_j \e_k^\intercal \|
%\]
%$\E[.] = p  \sum_\jk \w_\jk \u_j \e_k^\intercal $
%
%if consider Gaussian noise, then $\E[.] = 0$. try using:
%- first condition $\w_\jk$s and use matrix Bern. then uncondition . when applying matrix Bern $x_\jk  - \xstar_\jk$ is getting replaced by $\w_\jk$
%so
%\\
%$L = \max_\jk |\w_\jk| . \mu \sqrt{r/q} \sigmax$
%and
%$\sigma^2 = p \mu^2 (r/q) . \|\W\|_F^2 \le p \mu^2 (r/q) . (nq) \max_\jk |\w_\jk|^2 = np \mu^2 r  \max_\jk |\w_\jk|^2 $
%
%
%
%\subsection{Gradient term}
%\[
%GradNoise= \sum_\jk \zeta_\jk \w_\jk \e_j \b_k'
%\]


==> signalProcessingLetters/SPL_lrmc_altgdmin_Jain_proof_rewrite.tex <==

\clearpage

\subsection{Proof of Lemma \ref{lem:BerrLmma}: rewrite of the proof from Jain 2012 paper in our notation}
\label{subsec:BminG}
\[
\|\B - \G\|_F^2 = \|vec(\B - \G)\|^2
\]
We have $\b_k = \g_k + ( (\S_k \U)^\top (\S_k \U) )^{-1} \d_k$ where
\[
\d_k =  ( (\S_k \U)^\top \S_k  - (\S_k \U)^\top (\S_k \U) \U^\top  ) \Ustar \bstar_k
\]
Let $\D = [d_1 \mid \cdots \mid d_q]$, $z = [z_1 \mid \cdots \mid z_q]$, where $d_i,z_i$ are $r$-dimensional vectors, and $\U = [\u_1 \mid \cdots \mid \u_n]^\intercal \in \mathbb{R}^{n \times r}$.
Bound $\|\D\|_F = \|vec(\D)\|$ by using $\|vec(\D)\| = \max_{\| \z \| = 1 } \sum_k \z_k^\top \d_k $ and Lemma C.5 of Jain paper.
We need to bound
\[
\sum_k \z_k^\top \d_k =  \sum_k  \z_k^\top \M_k \bstar_k, \
\M_k:= ( (\S_k \U)^\top \S_k  - (\S_k \U)^\top (\S_k \U) \U^\top  ) = \sum_j \deltajk ({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)
\]

\[
 \z_k^\top \M_k \bstar_k = \sum_{l_1,l_2=1}^{l_1=r,l_2 = q} (\z_k)_{l_1} (\M_k)_{l_1l_2} (\bstar_k)_{l_2}
\]
and thus,
\[
\sum_k \z_k^\top \d_k = \sum_{l_1,l_2=1}^{l_1 = r, l_2 = q} \sum_k \sum_j \deltajk [ (\z_k)_{l_1} (\bstar_k)_{l_2} (({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar)_{l_1 l_2} ]
\]
We also have
\begin{equation}
\sum_j (({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar = (\U^\top - \U^\top \U \U^\top) \Ustar =   (\U^\top - \U^\top) \Ustar = \bm{0}_{r \times r} \label{eq:zroMtrx}
\end{equation}
%\textcolor{red}{ The above  is a summation over $r \times r$ matrices, not the  scalar entries of a vector; Lemma C.5 is for vectors.}
Lemma C.5 is applied to the sum of scalar entries $\sum_j [({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar]_{l_1l_2}$, which also has zero mean because
$$\sum_j [({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar]_{l_1l_2} =   [\sum_j({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar]_{l_1l_2} = 0 \enskip \because \eqref{eq:zroMtrx} $$
Thus we can apply Lemma C.5 to each $(p,q) \in [r,q]$-th entry of the summation and square both sides to get -- this use of $p,q$ is bad notation -- these are not the probability or the matrix dim q.
\[
 \left(\sum_k \sum_j \deltajk [ (\z_k)_{l_1} (\bstar_k)_{l_2} (({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar)_{l_1l_2}] \right)
\le \sqrt{q p} \sqrt{ \sum_k (\z_k)_{l_1}^2 (\bstar_k)_{l_2}^2 \sum_j  (({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar)_{l_1 l_2}^2 }
\]
and so wp at least $1 - 1/n^3$
\begin{align*}
\max_{\Z: \|\Z\|_F=1} \sum_k \z_k^\top \d_k
& \le \sum_{l_1,l_1} \sqrt{q p} \sqrt{ \sum_k (\z_k)_{l_1}^2 (\bstar_k)_{l_2}^2 \sum_j  (({\u^j} \e_j^\top  - {\u^j} {\u^j}^\top  \U^\top)\Ustar)_{l_1l_2}^2 }\\
& = \sqrt{q p} \sum_{l_1,l_2}  \sqrt{ \sum_k (\z_k)_{l_1}^2 (\bstar_k)_{l_2}^2 \sum_j  ({\u^j} (\e_j^\top  -  {\u^j}^\top  \U^\top)\Ustar)_{l_1l_2}^2 } \\
& = \sqrt{q p} \sum_{l_1,l_2}  \sqrt{ \sum_k (\z_k)_{l_1}^2 (\bstar_k)_{l_2}^2 \sum_j  ({\u^j})_{l_1}^2 (\e_j^\top  -  {\u^j}^\top  \U^\top)\Ustar)_{l_2}^2 } \\
& = \sqrt{q p} \sum_{l_1,l_2}  \sqrt{ \sum_k (\z_k)_{l_1}^2 (\bstar_k)_{l_2}^2 \sum_j  ({\u^j})_{l_1}^2 ((\e_j^\top  -  {\u^j}^\top  \U^\top)\Ustar)_{l_2}^2 } \\
& = \sqrt{q p} \sum_{l_1,l_2}  \sqrt{ \sum_k (\z_k)_{l_1}^2 (\bstar_k)_{l_2}^2 \max_j ({\u^j})_{l_1}^2 \sum_j  ((\e_j^\top  -  {\u^j}^\top  \U^\top)\Ustar)_{l_2}^2}\\
& \le \sqrt{q p} \sum_{l_1,l_2}  \sqrt{ \max_k (\bstar_k)_{l_2}^2 \sum_k (\z_k)_{l_1}^2  \max_j ({\u^j})_{l_1}^2 \sum_j  ((\e_j^\top  -  {\u^j}^\top  \U^\top)\Ustar)_{l_2}^2} \\
& \le \sqrt{q p} \sum_{l_1,l_2}  \max_k |\bstar_k|_{l_2}  \max_j |{\u^j}|_{l_1} \sqrt{  \sum_k (\z_k)_{l_1}^2  \sum_j  (\e_j^\top (\I  -  \U  \U^\top)\Ustar)^2_{l_2}} \\
&\le \sqrt{q p} \sum_{l_1,l_2}  \max_k |\bstar_k|_{l_2}  \max_j |{\u^j}|_{l_1} \sqrt{  \sum_k (\z_k)_{l_1}^2  \sum_j  \| \e_j^\top (\I  -  \U  \U^\top)\Ustar\|^2} \\
&  = \sqrt{q p} \sum_{l_1,l_2}  \max_k |\bstar_k|_{l_2}  \max_j |{\u^j}|_{l_1} \sqrt{  \sum_k (\z_k)_{l_1}^2 \SE_2(\U,\Ustar)^2} \\
& = \sqrt{q p} \sum_{l_1,l_2}  \max_k |\bstar_k|_{l_2}  \max_j |{\u^j}|_{l_1} \SE_2(\U,\Ustar) \sqrt{  \sum_k (\z_k)_{l_1}^2} \\
&  = \SE_2(\U,\Ustar)  \sqrt{q p}  \sum_{l_1,l_2}  \max_k |\bstar_k|_{l_2}    \max_j |{\u^j}|_{l_1} \sqrt{\sum_k (\z_k)_{l_1}^2} \\
& \le \SE_2(\U,\Ustar)  \sqrt{q p}   \sum_{l_1,l_2} \mu \sqrt{r/q} \sigmax   \mu_u \sqrt{r/n} \sqrt{\sum_k (\z_k)_{l_1}^2} \\
& \le \SE_2(\U,\Ustar)  \sqrt{q p} \cdot  \mu_u\mu \frac{r^2}{\sqrt{nq}} \sigmax   \sum_{l_1 = 1}^{l_1 = r}   \sqrt{\sum_k (\z_k)_{l_1}^2} &&  \\
& \le \SE_2(\U,\Ustar)  \sqrt{q p} \cdot  \mu_u\mu \frac{r}{\sqrt{nq}} \sigmax   \sum_{l_1 = 1}^{l_1 = r}   \|\Z^p\|   \\
&  \le \SE_2(\U,\Ustar)  \sqrt{q p} \cdot  \mu_u\mu \frac{r}{\sqrt{nq}} \sigmax   \sqrt{r} \|\Z\|_F   \ &&\text{$\Z^p$ is $p$-th row of $r \times q$ unit Frob norm $\Z$} \\
& = \SE_2(\U,\Ustar)  \sqrt{q p} \cdot  \mu_u\mu \frac{r}{\sqrt{nq}} \sigmax   \sqrt{r}   \\
& = \SE_2(\U,\Ustar)  \sqrt{q p} \cdot  \mu_u\mu \frac{r }{\sqrt{nq}} \sqrt{r}\sigmax     \\
& = \SE_2(\U,\Ustar)  \sqrt{p} \cdot  \mu_u\mu \frac{r }{\sqrt{n}} \sqrt{r}\sigmax     \\
& \le \delta^{(t)} \sqrt{r}\sigmax  \cdot \sqrt{p} \mu_u\mu \frac{r }{\sqrt{n}}
\end{align*}
Thus,
\[
\|\D\|_F \le   \delta^{(t)} \sqrt{r}\sigmax  \cdot \frac{\sqrt{p} \mu_u\mu  r }{\sqrt{n}}
\]
Also, by matrix Bernstein, w.p. {$1 - \exp(\log 2r - c \frac{n\eps^2p}{\mu_u\mu r}) $}, for fixed $r$.
\[
\|(\S_k \U)^\top (\S_k \U) - p \I\| \le \eps p
\]
Applying the union bound across $q$ terms and defining $F = BlockDiag( (\S_k \U)^\top (\S_k \U) ),  k \in [q]$, we have, {w.p. $1 - \exp(\log q + \log 2r - c \frac{n\eps^2p}{\mu_u\mu r}) ,$}
$$\| F^{-1} \|  \leq  \frac{1}{(1 - \epsilon)p} $$

and so $\sigma_{min}((\S_k \U)^\top (\S_k \U)) \ge (1-\eps) p =0.9 p$ if we set $\eps=0.1$. This bound is for a fixed $k$.

Let $F = BlockDiag( (\S_k \U)^\top (\S_k \U)), k \in [q]$.
\[
\|\B - \G\|_F = \|vec(\B - \G)\| = \| F^{-1} vec(\D) \| \le \frac{1}{0.9 p} \|\D\|_F \le C  \frac{\sqrt{p} \mu\mu_u  r }{\sqrt{n} p}  \delta^{(t)} \sqrt{r}\sigmax
\le C  \frac{\mu\mu_u  r }{\sqrt{np } }  \delta^{(t)} \sqrt{r}\sigmax,
\]
which is $\le  C \delta^{(t)} \sqrt{r}\sigmax$, assuming $p \ge \mu^2\mu_u^{2} r^2/n $.
%\subsection{Proof of Theorem \ref{thrm}. } %Try to show $\|\R^+{}^{-1}\| \le 1/ (1- \eta p \delta^{(t)} \sqrt{r} \sigmax^2) $ -- use same approach as in LRCS }
%\label{subsec:mainThm}
\section{Appendix}
\subsubsection{Lemma C.5 of Jain 2012 copied in our notation}
For two vectors $\z, \tilde\z$ of length $n,q$ respectively with $n \le q$, suppose that $\sum_j \z_j = 0$.
Suppose also that $p \ge C (\log q ) / n $.
Then w.p. at least $1 - 1/n^3$,
\[
| \sum_j \sum_k \deltajk \z_j \tilde\z_k  | \le C \sqrt{q p} \|\z\| \|\tilde\z\|
\]
\subsubsection{Matrix Bernstein inequality}


%\input{proof_lrmc_edit}


==> signalProcessingLetters/SPL_lrmc_altgdmin_proofs.tex <==

%\subsection{temp notes}
%?? use of $_2$ or do not use it -  be consistent.
%?? use of $\U$ -- remove $\hat\U$ or $\widehat\U$
%?? check required value of p by combining the 4 lemmas -- it seems to me it is r3 and not r4.5 for the iterations.
%
%Jain paper Lem C.2 shows that if $dist(U0,Ustar) < d_0$, then $dist(U0clip,Ustar) < C\sqrt{r d_0}$. To get this RHS to be below $1/\kappa \sqrt{r}$ we need $d_0 = 1/ \kappa^2 r^2$
%Lem C.1 shows that $dist(U0,Ustar) < C r \kappa / \sqrt{n p} $.  To get this RHS to be $1/r^2 \kappa^2$, we need $\sqrt{np} > r^3 \kappa^3$ or $np > r^6 \kappa^6$.
%%under assumed bound on p, $dist(U0,Ustar) < c/r$
%
%
%Lem C.6 : bounds $\U_k ' \U_k$
%
%Lem C.8 bounds $\B-\G$.

\appendices \onecolumn
%\appendix
\renewcommand\thetheorem{\Alph{section}.\arabic{theorem}}
\section{Main Lemmas and Proof of Theorem \ref{thrm}} \label{lemmas} %: Main Lemmas and Proof of Theorem using the Lemmas}

\subsection{Definitions}
%All lemmas assume that Assumption \ref{incoh} holds.
Recall that  $\delta^{(t)} = \SE_2(\U^{(t)},\U^*)$.
Let $\G \equiv \G^{(t)} = (\U^{(t)})^{\intercal}\Xstar$, $\U \equiv \U^{(t)}$, $\B \equiv \B^{(t+1)}$, and  $\X \equiv \X^{(t)} = \U^{(t)} \B^{(t+1)}$. Also let $\U^+ \equiv \U^{(t+1)}$.
Let $\xi_\jk \iidsim Bernoulli(p)$ for all $j \in [n], k \in [q]$. Thus $\Omega_k = \{j:  \xi_\jk = 1\}$ is the set of indices of the observed entries in column $k$. Recall that $\S_k = \I_{\Omega_k}{}^\intercal$ %is a $|\Omega_k| \times n$ 1-0 row selection matrix ($\S_k \M$ selects rows of $\M$ with indices in $\Omega_k$). %with exactly one 1 in each row corresponding to the index of the observed entry.
and $\U_k:=\S_k \U$. % where $\S_k = \I_{\Omega_k}{}^\intercal$ is a $|\Omega_k| \times n$ 1-0 matrix with exactly one 1 in each row corresponding to the index of the observed entry.
Let $\mu_u:= C\mu \sqrt r$.

%?? replace $\mu-star$ by $\mu$ everywhere.


\subsection{Lemmas}
All lemmas below assume Assumption \ref{incoh} (singular vectors' incoherence) holds.
\begin{lemma}(Initialization \cite[Lemma C.1 and C.2]{lowrank_altmin})
	\label{lem:init}
		%Let $\U^{(0)}$ be the initial iterate of Algorithm 1.
Assume $p \geq C \kappa^6 (\mu)^4 r^6 /n$. Then, w.p. at least $1 - 1/n^3$, we have
	\ben
	\item $\SE_2(\U^{(0)},\U^*) \leq c/(\sqrt{ r} \kappa^2).$
	\item $\U^{(0)}$ is incoherent with parameter $\mu_u:= C\mu \sqrt r$, that is, $\| {\u^j}^{(0)} \| \leq \mu_u\sqrt{\frac{r}{n}}$ for all $j \in [n]$.
	\een
	%	\textcolor{red}{For 2) to hold in Lemma \ref{lmma:init}, need subspace distance $\delta^{(0)} \leq c/r$. }
\end{lemma}

% $\| \v_k \| \leq \mu \sqrt{\frac{r}{q}}$,
%\begin{lemma}
%\cite[Lemma C.8]{lowrank_altmin}
%%	Let $\delta^{(t)} \triangleq \SE_2(\U^{(t)},\U^*)$.
%Assume $\| {\u^j} \| \leq \mu_u \sqrt{\frac{r}{n}}$ and  $p \geq  C \mu^2 \mu_u^2 r^2 \kappa^4/n$, $\delta^{(t)} < c/\sqrt{r} \kappa^2$. Then, w.p. greater than $1 - 1/n^3$,
%	\ben
%	\item $\| \B - \G  \|_F \leq \delta^{(t)} \sqrt{r} \sigma_{\max}^*$ \cite[Lemma C.8]{lowrank_altmin}.
%	\item This then implies that
%\ben
%\item $\| \X - \Xstar  \|_F \leq 2 \delta^{(t)} \sqrt{r} \sigma_{\max}^*$.
%	\item $\| \B \| \leq (1 + \delta^{(t)} \sqrt{r}) \sigma_{\max}^*$.
%	\item $\sigma_{\min}(\B) \geq  \sqrt{1 - \delta^{(t)^2}}\sigma_{\min}^*  - \delta^{(t)} \sigma_{\max}^*$.
%	\een
%\een
%	\label{lem:BerrLmma}
%	%where
%\end{lemma}

\begin{lemma}
\cite[Lemma C.8]{lowrank_altmin}
%	Let $\delta^{(t)} \triangleq \SE_2(\U^{(t)},\U^*)$.
Assume $\| {\u^j} \| \leq \mu_u \sqrt{\frac{r}{n}}$ and  $p \geq  C \mu^2 \mu_u^2 r^2 \kappa^4/n$, $\delta^{(t)} < c/\sqrt{r} \kappa^2$. Then, w.p. greater than $1 - 1/n^3$,
$\| \B - \G  \|_F \leq \delta^{(t)} \sqrt{r} \sigma_{\max}^*$.
	\label{lem:BerrLmma}
\end{lemma}

\begin{lemma}
%	Let $\delta^{(t)} \triangleq \SE_2(\U^{(t)},\U^*)$.
Assume $\| \B - \G  \|_F \leq \delta^{(t)} \sqrt{r} \sigma_{\max}^*$. Then,
\ben
\item $\| \X - \Xstar  \|_F \leq 2 \delta^{(t)} \sqrt{r} \sigma_{\max}^*$.
	\item $\| \B \| \leq (1 + \delta^{(t)} \sqrt{r}) \sigma_{\max}^*$.
	\item $\sigma_{\min}(\B) \geq  \sqrt{1 - \delta^{(t)^2}}\sigma_{\min}^*  - \delta^{(t)} \sigma_{\max}^*$.
	\een
	\label{Berr_implic}
	%where
\end{lemma}



%, and , where $\mu_u = C \kappa^2 \sqrt r \mu$,
\begin{lemma}
	\label{lem:BIncohLmma}
	Assume $\| {\u^j} \| \leq  \mu_u \sqrt{r/n}$ and  $p \geq C\frac{\mu_u^2 r}{n \epsilon^2 }(\log n  + \log r)$. Then, w.p. greater than  $1 - 1/n^3$,
%$1 - 	\exp(\log 2 r - c \frac{n \epsilon^2 p}{\mu_u^2 r})$,
%$\epsilon \leq 1$,
	$\| \b_k \| \leq 2 \sigma_{\max}^* \mu \sqrt{\frac{r}{q}}.$%
\end{lemma}



%$\| \B - \G  \|_F \leq \delta^{(t)} \sqrt r \sigma_{\max}^*$,
\begin{lemma}
	\label{lem:Ugrad}
	Assume  $\delta^{(t)} < c/\sqrt{r} \kappa^2$, $\| \B - \G  \|_F \leq \delta^{(t)} \sqrt r \sigma_{\max}^*$,
$\| {\u^j} \| \leq  \mu_u \sqrt{r/n}$, $\| \b_k \| \leq \sigmax\mu \sqrt{r/q}$, and $p \ge C \frac{\mu_u\mu}{n \eps^2} r(\log n + \log q)$.
Then,
	\ben
	\item $\| \gradU - \E[\gradU]  \| \leq \eps p \sqrt{r}  \delta^{(t)} \sigminTwo$ w.p. greater than $1 - 1/n^3$,  %$1 - \exp(\log q - \eps^2 p n  / \mu_u\mu r)$  $\forall \eps \leq 1$.
	\item $\E[\gradU] =  p (\X - \Xstar)\B^\intercal$ and so  $\|\E[\gradU]\| \leq p \sqrt{r} \delta^{(t)} \sigmaxTwo.$	
	\een
	\label{lemma:Ugrad}
	%	where $\U_j$ denotes the $j$-th row of matrix $\U$. \textcolor{red}{{Remove 3)} and make it part of incoherence Lemma \ref{lemma:Uincoh}.}
\end{lemma}

\begin{lemma}
	\label{lem:rowIncoh}
	Assume $\delta^{(t)} < c/\sqrt{r} \kappa^2$,  $\| \B - \G  \|_F \leq \delta^{(t)} \sqrt r \sigma_{\max}^*$, $\| \b_k \| \leq \sigmax \mu \sqrt{r/q}$, and $p \ge C  \mu^2 r \max(\log q, \log n )  / n$. Then, w.p. greater $1 - 1/n^3$,
	\ben
	\item $\| \gradUj - \E[\gradUj] \| \le 0.1 p  \|{\u^j}\|  \sigmaxTwo$ and %$1-\exp(\log q - \eps^2 p n / \mu^2\kappa^4 r )$.
	%\item $\| {\u^j}^{(t)}\| \leq \frac{3}{2}\tilde\mu \sqrt{\frac{r}{n}}, j \in [n], \,\, t \geq 0$, \, w.p. $1 - \exp(\log q - \eps^2 p n  / \tilde\mu^2 r)$  $\forall \eps \leq 1, \delta \leq c/\sqrt r \kappa^2$.
	\item %Assuming $\delta^{(t)} \leq  c/(\sqrt r \kappa^2)$, w.p. greater $1 - 1/n^3$,  %which requires $p> C (\mu)^{4}r^6\kappa^6/n$,  w.p. greater than $1 - \exp(\log q - \eps^2 p n / (\mu)^{2} \kappa^4 r ), \eps \leq 1$
$	
\|{\u^j}^{(t)}\|	\le  (1 - 0.15/\kappa^2)   \|({\u^j}^{(t-1)})\| +  0.7 \|{\ustar{}^j}\|.
$
	\een
\end{lemma}

%\begin{lemma}
%	\label{lem:rowIncoh}
%	Assume $\delta^{(t)} < c/\sqrt{r} \kappa^2$,  $\| \B - \G  \|_F \leq \delta^{(t)} \sqrt r \sigma_{\max}^*$, $\| \b_k \| \leq \sigmax \mu \sqrt{r/q}$, and $p > \kappa^4  \mu^2 r \max(\log q, \log n )  / n \eps^2$. Then, w.p. greater $1 - 1/n^3$,
%	\ben
%	\item $\| \gradUj - \E[\gradUj] \| \le \eps p  \|{\u^j}\|  \sigminTwo$ and %$1-\exp(\log q - \eps^2 p n / \mu^2\kappa^4 r )$.
%	%\item $\| {\u^j}^{(t)}\| \leq \frac{3}{2}\tilde\mu \sqrt{\frac{r}{n}}, j \in [n], \,\, t \geq 0$, \, w.p. $1 - \exp(\log q - \eps^2 p n  / \tilde\mu^2 r)$  $\forall \eps \leq 1, \delta \leq c/\sqrt r \kappa^2$.
%	\item %Assuming $\delta^{(t)} \leq  c/(\sqrt r \kappa^2)$, w.p. greater $1 - 1/n^3$,  %which requires $p> C (\mu)^{4}r^6\kappa^6/n$,  w.p. greater than $1 - \exp(\log q - \eps^2 p n / (\mu)^{2} \kappa^4 r ), \eps \leq 1$
%$	
%\|(\u^{(t)})^\intercal_j\|	\le  (1 - 0.15/\kappa^2)   \|({\u^j}^{(t-1)})^{\intercal}\| +  0.7 \|{\ustar{}^j}\|.
%$
%%Further, assuming $\delta^{(t')} \leq  c/(\sqrt r \kappa^2)$ for all $t'=0,1,\dots, t$, and assuming that $\| {\u^j}^{\intercal (0)} \| \leq C\sqrt{r}\mu  \sqrt{r/n}$, for $t \geq 0$,
%%	$$\|\u^{(t)}_j\| \leq C \mu_u \sqrt{r/n}, \,\,\, \mu_u = \kappa^2 \sqrt r \mu.$$
%	\een
%%$\| {\u^j}^{*\intercal} \| \leq \mu \sqrt{r/n}$,
%\end{lemma}



\begin{proof}%[Proofs of above lemmas] %This follows by combining Lemma \ref{lem:init} with the above theorem applied for each $t=1,2,\dots, T$.
The first two lemmas are taken from  \cite{lowrank_altmin}. The last four are proved using matrix Bernstein \cite[Theorem 5.4.1]{versh_book} and some linear algebra tricks borrowed from \cite{lrpr_gdmin}. The proofs are given in Appendix \ref{lemma_proofs} in longer version of this work \cite{lrmc_altgdmin_arxiv}.\end{proof}




\subsection{Proof of Theorem \ref{thrm}}
%assume $\delta^{(t)} \leq c/(\sqrt{r}\kappa^2)$ and that  $\U^{(t)}$ is $\mu_u$-incoherent.
%It is sufficient to analyze one iteration of the algorithm and show the following: i) $\delta^{(t+1)} \leq (1 - 0.5/\kappa^2) \delta^{(t)}$, ii) $\mu_u$-incoherence of $\U^{(t+1)}$.
%	\textit{Proof of \eqref{eq:SD_itr_bound}}.

We prove the following claim by induction. For all times $\tau \ge 0$, (i) $\delta^{(\tau)} \le c/\sqrt{r} \kappa^2$ and  $\delta^{(\tau)} \le (1 - c/ \kappa^2) \delta^{(\tau-1)}$;
(ii) $\|{\u^j}^{(\tau)}\| \le \mu_u \sqrt{r/n}$; (iii) $\|\B^{(\tau+1)} - \G^{(\tau+1)} \|_F \le \delta^{(\tau)} \sqrt{r} \sigmaxTwo$; and
(iv) $\|\b_k^{(\tau+1)} \| \le 1.1 \mu \sqrt{r/q} \sigmax.$
Theorem \ref{thrm} is the first claim of this result.


{\em Base case:} let  $\delta^{(-1)}=1$. Lemma \ref{lem:init} shows that $\delta^{(0)} \le c/\sqrt{r} \kappa^2$ and $\|{\u^j}^{(0)}\| \le C \sqrt{r} \mu \sqrt{r/n} = \mu_u \sqrt{r/n}$. Since $c/\sqrt{r} \kappa^2 < 1/2$, this implies that  $\delta^{(0)} \le  (1 - c/ \kappa^2) \delta^{(-1)}$. This proves (i) and (ii) for $\tau=0$. Lemmas  \ref{lem:BerrLmma} and \ref{lem:BIncohLmma} then prove (iii) and (iv) for $\tau=0$.%the two claims for $\B$.

{\em Induction assumption:} Assume the claim for $\tau=1,2, \dots, t$.


%This along with the base case then implies that $\delta^{(\tau)} \le c/\sqrt{r} \kappa^2$ for all $\tau=1,2,\dots, t$.

{\em Induction step:} We use the last five lemmas and the induction assumption to prove the claim for $\tau=t+1$.
%
%Using the expression for $\mu_u$,  $\eps=c$ if $p \ge C \kappa^4 \mu^2 r^3 \max(\log q, \log n) / n$.
%
The induction assumption implies that Lemma \ref{lem:rowIncoh} applies for all $\tau=1,2,\dots, t$. Using it and the base case,  $\|{\u^j}^{(0)}\| \le  \mu_u \sqrt{r/n}$ and  for all $\tau=1,2,\dots, t$,
\[	
\|{\u^j}^{(\tau)}\|	\le  (1 - 0.15/\kappa^2)   \|{\u^j}^{(\tau-1)}\| +  0.7 \|{\ustar{}^j}\|
\]
%for all $\tau=1,2,\dots, t$.
Applying this for each $\tau=0,1,\dots,t$,  % and using the base case,
$\|{\u^j}^{(t)} \| \le  (1 - \frac{0.15}{\kappa^2})^t \|{\u^j}^{(0)}\| + [1 + (1 - \frac{0.15}{\kappa^2})  + \dots + (1 - \frac{0.15}{\kappa^2})^{t-1}]  0.7 \|{\ustar{}^j}\|
 \le (1 - \frac{0.15}{\kappa^2})^t \|{\u^j}^{(0)}\|+ \frac{0.7 \kappa^2}{0.15} \|{\ustar{}^j}\|
 \le  \|{\u^j}^{(0)}\| + 5 \kappa^2 \|{\ustar{}^j}\|
 \le C \kappa^2 \sqrt{r}  \mu \sqrt{r/n} := \mu_u \sqrt{r/n}.
 $
%The last inequality follows using the base case bound on $\|{\u^j}^{(0)}\|$ and Assumption \ref{incoh}.
Thus, $\|{\u^j}^{(t)}\| \le \mu_u \sqrt{r/n}$, i.e. (ii) holds for $\tau=t$.

Using this and the induction assumption bound on $\|\B - \G\|_F$ and $\|\b_k\|$ for $\tau=t$, Lemma \ref{lem:Ugrad} applies. Using it, $\E[\gradU] =  p (\U\B - \Xstar)\B^\intercal$,  $\|\E[\gradU]\| \leq p \sqrt{r} \delta^{(t)} \sigmaxTwo$, and, if $p \ge C \frac{\mu_u\mu r}{n \eps^2} (\log n + \log q)$, then $\| \gradU - \E\gradU \| \leq \eps p \sqrt{r} \delta^{(t)}\sigmaxTwo$. Set $\eps = 0.1/\sqrt{r} \kappa^2$.
Then,  $\| \gradU - \E\gradU \| \leq  0.1 p \delta^{(t)} \sigminTwo$  if $p \ge C \frac{\kappa^4 \mu_u\mu r^2}{n}(\log n + \log q)$,
We use this to bound
$\delta^{(t+1)} := \SE_2(\U^+,\U^*)$ is bounded as follows.
%Let $\U^+  = \U^{(t+1)}$ and $\U = \U^{(t)}$.
Let $\P := \I - \Ustar \Ustar^\top, \text{ thus } \P \Xstar = \bm{0}$. Recall that $\|\P\U\| = \delta^{(t)}$, $\tilde\U^+ = \U - \eta \gradU$, and $\U^+ =\tilde\U^+ \R^+{}^{-1}$ where $\tilde\U^+ \qreq \U^+ \R^+$. We have
%\|\P (\U - \eta \gradU)\|
\begin{align}
\delta^{(t+1)} & =   \SE_2(\U^+, \Ustar)
	 = 	 \| \P \U^+ \| \notag\\
	& \le     \|\P \tilde\U^+\| \cdot \|(\R^+)^{-1}\| =  \|\P \tilde\U^+\|/\sigma_{\min}(\tilde\U^+)  \notag\\
	& \le   \frac{\|\P (\U - \eta \E[\gradU] + \eta \E[\gradU] - \eta \gradU)\|}{(1 - \eta \|\gradU\|)} \notag \\
%& \le  \frac{\|\P (\U - \eta \E[\gradU] + \eta \E[\gradU] - \eta \gradU)\|}{(1 - \eta \|\E[\gradU]  - \E[\gradU] +  \gradU \|)}\notag  \\
	& \le  \frac{\|\P (\U - \eta p(\U \B - \Xstar)\B^\top)\| + \eta \|\E[\gradU] - \gradU)\|}{(1 - \eta \|\E[\gradU]\| - \eta \| \E[\gradU] - \gradU\|)}\notag \\
	& \le  \frac{\|\P \U\| \cdot \|(\I - \eta p \B \B^\top) \| + \eta \|\E[\gradU] - \gradU)\|}{(1 - \eta \|\E[\gradU]\| - \eta \| \E[\gradU] - \gradU\|)}.
	\label{eq:SD_interm}
\end{align}
%where we used $\P \Xstar = \bm{0}$ and  $\|\P\U\| = \delta^{(t)}$. %We next use the bounds from Lemma \ref{lem:Ugrad}.
%
%As argued in the proof of Lemma \ref{lem:rowIncoh},
Since $\delta^{(t)} \leq c/(\sqrt{r}\kappa^2)$, using the induction assumption and Lemma \ref{Berr_implic}, $\sigma_{\min}(\B) \ge 0.9\sigmin$ and $\|\B\|\le 1.1 \sigmax$. Using these, if $\eta \leq 0.5/(p\sigmaxTwo)$, then $\I - \eta p \B\B^\intercal$ is positive semi-definite (psd) and $\| \I - \eta p \B\B^\intercal \| \leq 1 - 0.8 \eta p \sigminTwo$ (see details in proof of Lemma \ref{lem:rowIncoh}).
Using this and the bounds from Lemma \ref{lem:Ugrad}  in \eqref{eq:SD_interm}, and using ${1}/{(1 - x)} \leq 1 + 2x$ for $x<0.5$,% we have:
{\small
\begin{align*} %
\delta^{(t+1)}
%& = \SE (\U^{(t+1)}, \Ustar)  \\
& \leq  \frac{\delta^{(t)}\big(1 - 0.8\eta p\sigminTwo +  0.1 \eta p \sigminTwo \big)}{ 1 - \delta^{(t)}\big( (1 + \eps) \eta p \sqrt r \sigmaxTwo \big)}\notag\\
 &\leq \delta^{(t)} (1 - 0.7\eta p\sigminTwo) (1 + 2 \delta^{(t)}( (1 + \epsilon) \eta p \sqrt r \sigmaxTwo )) \label{eq:Ceqn}\\
	&\leq \delta^{(t)}  (1 - 0.7 \eta p\sigminTwo   +  \delta^{(t)} \cdot 2(1 + \epsilon) \eta p \sqrt r \sigmaxTwo  ) \\
	&\leq \delta^{(t)}  (1 - \eta p\sigminTwo (0.7 - \delta^{(t)}  2(1 + \epsilon)\sqrt{r} \kappa^2 ) ) \\
	&\leq \delta^{(t)}  (1 - \eta p\sigminTwo (0.7 - 0.1 ) )
	%&\leq &&  \delta^{(t)}\big(1  + \eta \eps p \sqrt r \sigmaxTwo - \eta p \sigminTwo(\cdots \notag\\
%	&  &&0.8 - C\delta^{(t)}(1 + \eps)\sqrt r \kappa^2 - C \delta^{(t)}\eps(1 + \eps) \eta^2 p^2 r \kappa^2 \sigmaxTwo ) \big). \label{eq:SDexprsn}
\end{align*}
}
%if $\delta^{(t)} \leq 0.1/(\sqrt{r}\kappa^2)$ and $\eta \leq 0.5/(p\sigmaxTwo)$,
%In the last inequality we used $\delta^{(t)} < c/\sqrt{r} \kappa^2$.
The last row used $\delta^{(t)} \leq 0.1/(\sqrt{r}\kappa^2)$.
Setting $\eta = 0.5/(p\sigmaxTwo)$,
$
\delta^{(t+1)} \le (1 - 0.3/ \kappa^2) \delta^{(t)}.
$
Using this and the induction assumption, $\delta^{(t+1)} \le c/ \sqrt{r} \kappa^2$. Thus claim (i) holds.
Using Lemmas \ref{lem:BerrLmma} and \ref{lem:BIncohLmma}, claims (iii) and (iv) hold.%
%$\|\B^{(t+2)} - \G^{(t+2)} \|_F \le \delta^{(t+1)} \sqrt{r} \sigmaxTwo$ and $\|\b_k^{(t+2)} \| \le 1.1 \mu \sqrt{r/q} \sigmax$.

%\clearpage \onecolumn


\section{Proofs of Corollary \ref{corollary} and the Lemmas}\label{lemma_proofs}
\subsection{Proof of Corollary \ref{corollary}}
\begin{proof}  	
	By Lemma \ref{lem:init},  if $p \geq C \kappa^6 (\mu)^4 r^6 /n$, then $\delta^{(0)} \leq c/(\sqrt{r}{\kappa^2})$ and $\U^{(0)}$ is $\mu\sqrt{r}$-incoherent. Applying the Theorem for each $t=1,2,\dots, T$, we can conclude that if $p \geq C \kappa^6 (\mu)^4 r^{4.5} (r^{1.5} + T) / n$, then $\SE_2(\U^{(T)},\U^*)  \le (1 - 0.5/\kappa^2)^T \cdot c/(\sqrt{r}{\kappa^2})$. Using the value of $T$, this right hand side is below $\eps$. The bound on $\|\X^{(T)} - \Xstar\|_F $ then follows using Lemmas \ref{lem:BerrLmma} and \ref{Berr_implic}.
\end{proof}


\subsection{Brief proof ideas}

Lemma \ref{Berr_implic} is proved below.

Lemma \ref{lem:BIncohLmma} follows  by writing $\b_k = (\U_k^\intercal\U_k)(\U_k^\intercal\U^*_k) \b^*_k$ applying the Matrix-Bernstein inequality twice to bound $\| \U_k^\intercal\U_k \|$ and $\U_k^\intercal\U^*_k$. See section \ref{subsec:bkIncoh}.

Lemma \ref{lemma:Ugrad}:  For 1), we use the Matrix Bernstein inequality, see section \ref{subsec:gradUBnd}.
	For 2), note that $ \E[\gradU]  =   p (\X - \Xstar)\B^\intercal$ because the expectation is taken with respect to an independent set of samples at each iteration, i.e., sample splitting. %The bound then follows using Lemma \ref{lem:BerrLmma}.
%THIS IS WRONG Subsequently, $\| \E[\gradU] \| = p \| (\I - \U\U^\intercal)\U^* \B^* \| \leq p \| (\I - \U\U^\intercal) \U^*\| \| \B^* \| \leq p\delta \sigmax.$


Lemma \ref{lem:rowIncoh}: 	1) follows by using the Matrix-Bernstein inequality. For 2), we write $\tilde{\u}^{j^{(t+1)}} =  {\u^j}^{(t)}  - \eta\gradUj \pm \E[\gradUj]$ and subsequently bounding $ \| {\u^j}^{\intercal(t+1)} \| \leq \| \R^{-1 } \|  \| \tilde{\u}^{j^{(t)}} \|$. The proofs are provided in Section \ref{subsec:rowIncohProof}.


\subsection{Proof of Lemma \ref{Berr_implic}}
%	1) The bound on $\| \B - \G \|$ is proven in \cite{lowrank_altmin}. %See  Section \ref{subsec:BminG} for a reproduction of the original proof in our notation.
Writing $\Xstar = \U\G + (\I - \U\U^\intercal)\Xstar$, and $\X = \U \B$, we have
	$
	\| \Xstar - \X \|_F %\leq \| \U(\G-\B)  + (\I - \U\U^\intercal)\Xstar  \|_F
\leq
	\| \B - \G \|_F  + \| (\I - \U\U^\intercal)\U^*\B^* \|_F\leq
	\| \B - \G \|_F + \| (\I - \U\U^\intercal)\U^*\|_F  \| \B^* \| \leq
	\delta^{(t)} \sqrt r \sigma_{\max}^* + \delta^{(t)} \sqrt r \sigma_{\max}^*.
	$

	For the second part, using the bound on $\| \B - \G \|$, $\| \B \| = \| \B - \G   + \G \| \leq \| \B - \G \| + \| \G \| \leq  \delta^{(t)} \sqrt r \sigma_{\max}^* + \sigma_{\max}^*.$ 	

	For the third part, $\sigma_{\min}(\B)\geq \sigma_{\min}(\G) - \sigma_{\max}(\B -\G) \geq \sqrt{1 - \delta^{(t)^{2}}}\sigma_{\min} -\delta^{(t)} \sqrt r \sigma_{\max}^*$, where $\sigma_{\min}(\G) = \sigma_{\min}(\U^\intercal \U^*\B^*) \geq \sigma_{\min}(\U^\intercal \U^*) \sigma_{\min}^* \geq \sqrt{1 -\delta^{(t)^2}}\sigma_{\min}^*.$



\subsection{Proof of Lemma \ref{lemma:Ugrad}}
\label{subsec:gradUBnd}
The gradient with respect to $\U$ is
$\gradU = \sum_{jk}  \deltajk \e_j (\x_{jk} - \x^*_{jk})\b_k^\intercal.$
We will bound $\| \gradU \|$ by the Matrix-Bernstein inequality. Using $n \le q$ and \eqref{eq:elmntErrBnd},
\[
L = \max_\jk |\x_\jk - \xstar_\jk|  \max_k \|\b_k\| \le   2\mu_u (r/\sqrt{n})  \delta^{(t)} \sigmax \cdot \mu \sqrt{r/q} \sigmax \le  2\mu_u \mu (r^{3/2} / n) \delta^{(t)} \sigmaxTwo,
\]
where $\max_{jk} |\x_{jk} - \x^*_{jk}|$ is bounded below
\begin{align}
	|\e_j^\top(\X - \Xstar)\e_k| % = |\e_j^\top(\U (\B - \G) + (\U \U^\top \Xstar - \Xstar) )\e_k|
	\le  \|\e_j^\top\U \| \|\B - \G\| + \|(\U \U^\top - \I)\Ustar\| \|\Bstar \e_k\|
	\le \mu_u \sqrt{r/n} \sqrt{r} \delta^{(t)} \sigmax + \mu \sqrt{r/q} \delta^{(t)}  \sigmax
	\le 2 \mu_u (r/\sqrt{n}) \delta^{(t)} \sigmax.
	\label{eq:elmntErrBnd}
\end{align}
The variances are
\begin{align}
&\sigma_1^2
= p \sum_\jk (\x_\jk - \xstar_\jk)^2 \e_j \b_k^\top \b_k \e_j^\top %\le p \cdot q \cdot \tilde\mu^2 (r^2/n) \cdot \tilde\mu^2 (r/q) \delta^{(t)}{}^2 \sigmax^4 =  p \cdot \tilde\mu^4 (r^3/n) \delta^{(t)}{}^2 \sigmax^4
%\le p \|\b_k\|^2 \cdot \|\e_j\|^2 \sum_\jk (\x_\jk - \xstar_\jk)^2
\le  p \|\b_k\|^2 \|\X - \Xstar\|_F^2
\le p\mu^2(r/q) \sigmaxTwo \cdot  ( \delta^{(t)} \sqrt{r} \sigmax )^2
= p\mu^2(r^2/q) \delta^{(t)}{}^2 \sigmax^4. \notag\\
&\sigma_2^2
= p \| \sum_\jk (\x_\jk - \xstar_\jk)^2 \e_j^\top \e_j \b_k\b_k^\top \|
%\le p \|\b_k\|^2 \| \sum_\jk (\x_\jk - \xstar_\jk)^2 \|
\le  p \|\b_k\|^2 \|\X - \Xstar\|_F^2  = \sigma_1^2. \notag
\end{align}
Setting $t = \eps p \sqrt{r}  \delta^{(t)} \sigmaxTwo $, we have
\[
\frac{t^2}{\sigma^2} = \frac{\eps^2 p^2 r \delta^{(t)}{}^2 \sigmax^4}{p \mu^2(r^2/q) \delta^{(t)}{}^2 \sigmax^4}  = \frac{\eps^2 p q}{\mu^2 r} \leq \frac{\eps^2 p q}{\mu_u\mu r},
\ \
\frac{t}{L} = \frac{ \eps p \sqrt{r}  \delta^{(t)} \sigmaxTwo}{\mu_u\mu (r^{3/2} / n) \delta^{(t)} \sigmaxTwo} =  \frac{ \eps p n }{\mu_u\mu r}.
\]
By matrix Bernstein, for $\eps \leq 1$, w.p. at least $1 - \exp(\log q - \eps^2 p n  /\mu_u \mu r) $,
\[
\|\gradU - \E[\gradU] \| \le \eps p \sqrt{r}  \delta^{(t)} \sigmaxTwo.
\]
If $p > \mu_u \mu r \max(\log q, \log n )  / n \eps^2$, then the above bound holds w.p. at least $1 - 1/n^3$. Also,
\[
\E[\gradU] = p (\X- \Xstar) \B^\top,  %\ \ \|\E[\gradU] \| \le p \sqrt{r} \delta^{(t)} \sigmaxTwo.
\]

\subsection{Proof of Lemma \ref{lem:rowIncoh}}
\label{subsec:rowIncohProof}
% \le\max( \|{\u^j}\|, \|{\ustar{}^j}\|) \max(\|\b_k\|^2, \|\bstar_k\| \cdot \max_k \|\b_k\|)
Let $\gradUj \in \mathbb{R}^{1 \times r}$ denote the gradient of $\U \in \mathbb{R}^{n \times r}$ with respect to row $j$. We note the following
\begin{align}
& \gradUj = \sum_k \deltajk (\x_\jk - \xstar_\jk) \b_k^\top,
%\E[\gradU_j] = p \e_j^\top(\U \B \B^\top - \Ustar \Bstar \B^\top) ,
\ \|\E[\gradU_j] \| \lesssim 2 p \|{\u^j}\|  \sigmaxTwo.\notag\\
& L =  \max_k |\x_\jk - \xstar_\jk| \max_k \|\b_k\|  \le  \max( \max_k |\x_\jk| , \max_k |\xstar_\jk|) \max_k \|\b_k\|  \le   \max( \|{\u^j}\|, \|{\ustar{}^j}\|)  \mu^2 (r/q) \sigmaxTwo. \notag\\
& \sigma_1^2
= \| \sum_k p (\x_\jk - \xstar_\jk)^2 \b_k^\top \b_k \|
\le  2p \| \sum_k {\u^j}^\top \b_k \b_k^\top {\u^j}  \b_k^\top \b_k \| \le 2p \max_k \|\b_k\|^2  {\u^j}^\top (\sum_k \b_k \b_k^\top ) {\u^j}
\le 2p  \|{\u^j}\|^2 \mu^2 (r/q) \sigmax^4. \notag \\
&\sigma_2^2
= \| \sum_k p (\x_\jk - \xstar_\jk)^2 \b_k\b_k^\top \|
\le  2p \|  \sum_k {\u^j}^\top \b_k \b_k^\top {\u^j}  \b_k\b_k^\top \|  \le   2p\max_k \| \b_k\|^2  \| {\u^j}^\top (\sum_k \b_k \b_k^\top ) {\u^j} \| \notag \le 2p  \|{\u^j}\|^2 \mu^2 (r/q) \sigmax^4. \notag
\end{align}
Here, $\sigma_1^2 \equiv \E[\sum_k \deltajk (\x_{jk} - \x^*_{jk})^2\b_k^\intercal\b_k]$
and $\sigma_2^2 \equiv \E[\sum_k \deltajk (\x_{jk} - \x^*_{jk})^2\b_k\b_k^\intercal]$. By the matrix Bernstein inequality with $t = \eps p  \|{\u^j}\|  \sigminTwo$, we have
w.p. at least  $1 - \exp(\log q - \eps^2 p n /\mu^2 \kappa^4 r )$,
\[
\|\E[\gradU_j] - \gradU_j \| \le \eps p  \|{\u^j}\|  \sigminTwo.
\]
This completes the proof for the first part of the lemma.

By line 5 of Algorithm 1, adding/subtracting $\E[\gradU_j] = p {\ustar{}^j}{}^\top  \Bstar \B^\top$, and using the above bound on $\|\E[\gradU_j] - \gradU_j \|$
\[
\tilde{\u}^{(t+1)^\top}_j  =
%\R^{-1}
 {\u^j}^{(t)\top}  ( \I - \eta p \B \B^\top) - \eta \gradU_j =  {\u^j}^{(t)\top}  ( \I - \eta p \B \B^\top)
 - \eta p {\ustar{}^j}{}^\top  \Bstar \B^\top + \eta (\E[\gradU_j] - \gradU_j),
\]
w.p. at least $1 - \exp(\log q - \eps^2 p n /\mu^2 \kappa^4 r )$.

Using the assumed bound on $\B-\G$ and Lemma \ref{Berr_implic} and  $\delta^{(t)} \leq c/\sqrt{r}\kappa^2$, $\sigma_{\min}(\B) \ge 0.9 \sigmin$ and $\sigma_{\max}(\B) \le 1.1 \sigmax$. Thus, if  $\eta < 0.5 / p \sigmaxTwo$ then, $\I - \eta p \B \B^\top$ is positive semi-definite (psd) and $\|\I - \eta p \B \B^\top\|  = 1 - \eta p \sigma_{\min}^2(\B) \leq  1 - 0.9 \eta p \sigminTwo$. Thus, if  $\eta < 0.5 / p \sigmaxTwo$, then,
\begin{equation}
\|\tilde{\u}^{(t+1)}_j \|
\le \|{\u^j}^{(t)}\| (1 - 0.9\eta p \sigminTwo) + \eps \eta p \sigminTwo \|{\u^j}^{(t)}\|   + 1.1 \eta p \|{\ustar{}^j}\| \sigmaxTwo
\le  (1 - (0.9-\eps)\eta p \sigminTwo )\|{\u^j}^{(t)}\|    + \eta p \sigmaxTwo \|{\ustar{}^j}\|.
\label{eq:uTildeBnd}
\end{equation}
w.p. at least $1 - \exp(\log q - \eps^2 p n /\mu^2 \kappa^4 r )$.

We bound $\| {\u^j}^{\intercal (t+1)} \| \leq  \| (\R^{(t+1)})^{-1} \| \cdot \| \tilde{\u}^{\intercal (t+1)}_j \|$, where $\tilde \U^{(t+1)} \overset{\text{QR}}{=} \U^{(t+1)} \R^{(t+1)} $, and
\begin{equation}
	\| (\R^{(t+1)})^{-1} \| = 1/(\sigma_{\min}(\U - \eta  \| \gradU \| )
	\leq  1/(1 - \eta p (1 + \epsilon) \sqrt{r} \delta^{(t)} \sigma_{\max}^{*2})
	\leq 1/(1 - 0.25\eta p  \sigminTwo)
	\leq 1 + 0.5 \eta p  \sigminTwo.  \label{eq:RinvBnd}
\end{equation}
w.p. given in Lemma \ref{lemma:Ugrad}.  In the above we have used Lemma \ref{lemma:Ugrad} and the upper bound on $\delta^{(t)}$. Thus,
\begin{align*}
\|{\u}^{(t+1)}_j \|
& \le (1 + 0.5 \eta p  \sigminTwo) (1 - (0.9-\eps) \eta p \sigminTwo ) \|{\u^j}^{(t)}\| + (1 + 0.5 \eta p  \sigminTwo) \eta p \sigmaxTwo \|{\ustar{}^j}\| \\
& \le (1 - (0.4-\eps) \eta p \sigminTwo ) \|{\u^j}^{(t)}\| + (1 + 0.5 \eta p  \sigminTwo) \eta p \sigmaxTwo \|{\ustar{}^j}\| \\
& \le (1 - (0.4-\eps) \eta p \sigminTwo ) \|{\u^j}^{(t)}\| + (1 + 0.25/\kappa^2) 0.5 \|{\ustar{}^j}\| \\
& \le (1 - \frac{0.15}{\kappa^2}) \|{\u^j}^{(t)}\| + 0.7 \|{\ustar{}^j}\|
\end{align*}
where the last bound follows by setting $\eta = 0.5/p \sigmaxTwo$, $\eps=0.1$.

Thus, we have shown that if $\delta^{(t)} \leq c/\sqrt{r}\kappa^2$, and $\eta = 0.5/p \sigmaxTwo$,   w.p. at least $1 - 3/n^3$,
\[
\|{\u^j}^{(t+1)} \|  \le (1 - \frac{0.15}{\kappa^2}) \|{\u^j}^{(t)}\| + 0.7 \|{\ustar{}^j}\|
\]
if $p$ satisfies the stated bound in the lemma.

%\subsubsection{delete}
%Assuming the above bound on $\delta^{(t')}$ for all $t'=0,1,\dots, t$, we can use the above equation at each $t'$ to argue that
%\begin{align*}
%\|{\u}^{(t+1)}_j \|
%& \le (1 - \frac{0.15}{\kappa^2})^t \|{\u^j}^{(0)}\| + [1 + (1 - \frac{0.15}{\kappa^2}) + (1 - \frac{0.15}{\kappa^2})^2 + \dots + (1 - \frac{0.15}{\kappa^2})^t]  0.7 \|{\ustar{}^j}\| \\
%& \le (1 - \frac{0.15}{\kappa^2})^t \|{\u^j}^{(0)}\|+ \frac{0.7 \kappa^2}{0.15} \|{\ustar{}^j}\|
%\le  \|{\u^j}^{(0)}\| + 5 \kappa^2 \|{\ustar{}^j}\| \le C \kappa^2 \sqrt{r}  \mu \sqrt{r/n}
%\end{align*}
%where for the last bound we used $\|{\u^j}^{(0)}\| \le C \sqrt{r} \mu \sqrt{r/n}$ and Assumption \ref{incoh}



\subsection{Proof of Lemma \ref{lem:BIncohLmma}}
\label{subsec:bkIncoh}
	We have
	\begin{equation}
		\b_k = \underbrace{(\U_k^\intercal\U_k)^{-1}}_{T_1} \underbrace{\U_k^\intercal \U_k^*}_{T_2} \b^*_k.
		\label{eq:bk}
	\end{equation}

The following has been proved in Lemma C.6 of  \cite{lowrank_altmin}.
If $p \geq C\frac{\mu_u^2 r}{n \epsilon^2 }(\log n  + \log r)$, then  with probability greater than $1 - \frac{1}{n^3}$,
	\begin{equation}
		\| (\U_k^\intercal \U_k)^{-1} \| \leq  \frac{1}{(1 - \epsilon)p}. \label{eq:opBndTrm1Fnl}
	\end{equation}
	%Similar to \eqref{eq:lbdMin}, we also have
	%\begin{equation}
	%	\lambda_{\min} \leq p + \| \U_k\U_k^\intercal - p \I \|,
	%\end{equation}
	%which gives the two-sided bound: w.h.p and $\epsilon \leq 2$,
	%\begin{equation}
	%	\frac{1}{(1 + \epsilon)p} \leq \| (\U_k\U_k^\intercal)^{-1} \| \leq \frac{1}{(1 - \epsilon)p}.
	%	\label{eq:T1_2sided}
	%\end{equation}


Consider the second term, $T_2$.  The term $\| T_2 - \E[T_2] \|$ can be bounded by the Matrix-Bernstein inequality.
	We have $\E[T_2] = p \U^\intercal \U^* \neq p \I$. By the reverse triangle inequality,
	\begin{align}
		\| \U_k^\intercal \U_k^* - p \U^\intercal \U^* \|	 \geq \| \U_k^\intercal \U_k^* \| - p,
	\end{align}
	where we have used $\| \U^\intercal \U^* \| \leq \| \U \| \| \U^* \| \leq 1$. Therefore,
	\begin{equation}
		\| \U_k^\intercal \U_k^* \| \leq \| \U_k^\intercal \U_k^* - p \U^\intercal \U^* \|_{op } + p.
		\label{eq:rvsTrngleIcoh}
	\end{equation}
	The second difference from the proof of  \eqref{eq:opBndTrm1Fnl} is that $T_2 - \E[T_2]$ is not symmetric. The variance $\sigma^2$ is now
	$$\sigma^2 = \max(\| \sum_j \E [\Z_j \Z_j^\intercal] \|, \| \sum_j \E[\Z_j^\intercal \Z_j]\| ),$$
	where $\Z_j = (\deltajk - p){\u^j} {\u^j}^{*\intercal}$, and
	\begin{align}
		&\E[\Z_j] = 0 \notag,\\
		&\|  \Z_j \| = \max(1-p,p) \| {\u^j} \| \| {\u^j}^* \| \leq \mu_u\mu \frac{r}{n}, \notag\\
		& \Z_j\Z_j^\intercal \sim
		\begin{cases}
			(1-p)^2 \| {\u^j}^* \|^2 {\u^j} {\u^j}^\intercal  & \text{w.p. } p\\
			p^2 \| {\u^j}^* \|^2 {\u^j} {\u^j}^\intercal & \text{w.p. } 1-p,
		\end{cases} \notag\\
		& \Z_j^\intercal \Z_j \sim
		\begin{cases}
			(1-p)^2 \| {\u^j} \|^2 {\u^j}^* {\u^j}^{*\intercal}  & \text{w.p. } p\\
			p^2 \| {\u^j} \|^2 {\u^j}^{*} {\u^j}^{*\intercal} & \text{w.p. } 1-p,
		\end{cases} \notag
		%	& p' = p(1-p)^2 + p^2(1-p) \leq 2p. \notag
		%& \| \sum_{j=1}^{j=n} \E[\X^2_j] \| =  p' \|   \sum_{j=1}^{j=n} \| {\u^j} \|^2  ({\u^j} {\u^j}^\intercal) \| \leq 2p \tilde\mu^2 \frac{r}{n}. \label{eq:varBndT2}
	\end{align}
	%The bound on the variance $\sigma^2$ in \eqref{eq:varBndT2} follows from
	Both variances $\sigma^2(\Z_j \Z_j^\intercal)$ and $\sigma^2(\Z_j^\intercal \Z_j)$ can be bounded by the same upper bound. Note that \begin{align}
		\E[\Z_j\Z_j^\intercal] &= p(1-p)^2 \| {\ustar{}^j} \|^2 {\u^j}{\u^j}^\intercal + p^2(1-p)\| {\ustar{}^j} \|^2 {\u^j} {\u^j}^\intercal \notag \\ &\triangleq p' \| {\u^j}^* \|^2 {\u^j} {\u^j}^\intercal,  \enskip \text{ where }  p' = p(1-p)^2 + p^2(1-p) \leq 2p.  \end{align}
	The variance $\sigma^2(\Z_j \Z_j^\intercal)$ is
	\begin{align}
		\sigma^2(\Z_j \Z_j^\intercal)	& =  \| \sum_{j=1}^{j=n} \E[\Z_j\Z_j^\intercal] \| =  p' \|   \sum_{j=1}^{j=n} \| {\u^j}^* \|^2   ({\u^j} {\u^j}^\intercal) \| \notag \\
		&= p' \max_{\w \colon \| \w \| = 1}  \sum_{j=1}^{j=n} \w^\intercal (\| {\u^j}^* \|^2 {\u^j} {\u^j}^\intercal) \w \notag \\
		&\leq p' \mu^2 \frac{r}{n} \max_{\w \colon \| \w \| = 1} \w^\intercal  \sum_{j=1}^{j=n}   {\u^j} {\u^j}^\intercal \w \notag \\
		&\leq p' \mu^2 \frac{r}{n} \max_{\w \colon \| \w \| = 1} \w^\intercal  \U^\intercal\U \w \notag\\
		& = p' \mu^2\frac{r}{n} \max_{\w} \w^\intercal \w \notag \\
		&= p' \mu^2 \frac{r}{n} \leq 2p \mu^2 \frac{r}{n} \notag.
	\end{align}
	$\sigma^2(\Z_j^\intercal \Z_j)$ can be similarly bounded as $\sigma^2(\Z_j^\intercal \Z_j) \leq 2p \mu_u^{2}\frac{r}{n}$. Because $\mu_u \geq \mu$, we have $\sigma^2(\Z_j \Z_j^\intercal) \geq \sigma^2(\Z_j^\intercal \Z_j)$. %Analogous to \eqref{eq:T1EpsBnd},
By the Matrix-Bernstein inequality, for $\epsilon \leq 2$ and w.p. greater than $1 - \exp(\log 2 r - c \frac{n \epsilon^2 p}{\mu_u^2 r})$
	\begin{equation}
		\| \U_k^\intercal \U_k^* - p \U^\intercal \U^* \| \leq \epsilon p.
		\label{eq:mtrxBrnstnIncoh}
	\end{equation}
	From \eqref{eq:rvsTrngleIcoh} and \eqref{eq:mtrxBrnstnIncoh},  w.h.p,
	\begin{equation}
		\| \U_k^\intercal \U^*_k \| \leq (1 + \epsilon)p. \label{eq:T2_incoh_bnd}
	\end{equation}
	Substituting \eqref{eq:opBndTrm1Fnl},  \eqref{eq:T2_incoh_bnd} in \eqref{eq:bk}, and setting $\epsilon =1/10$, we have
	\begin{equation}
		\| \b_k \| \leq \frac{3}{2} \| \b^*_k \| \leq \frac{3}{2} \sigma_{\max}^* \mu \sqrt{r/q}.
	\end{equation}


==> signalProcessingLetters/SPL_lrmc_altgdmin_sims.tex <==

\vspace{-0.1in}
\section{Simulation Results}
\label{sec:results}
\begin{figure}
%	\centering
%	\begin{subfigure}{0.45\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{fig3.pdf}
%		\caption{}
%		\label{fig:errAgnstIterr10}
%	\end{subfigure}
	%\begin{subfigure}{0.71\linewidth}
		\centering
		\includegraphics[width=0.75\linewidth]{figTruncNew.pdf}
%		\caption{}
		\label{fig:errAgnstTimer10}
	%\end{subfigure}
\vspace{-0.1in}
	\caption{\small{Comparison with benchmarks. Smaller figure compares AltGDMin with second fastest benchmark, AltMin(Fed./NotPrvt.)}.%
%See Section \ref{sec:results} for an explanation of the results and  Sec. \ref{sec:bnchmrks} for a description of the benchmark methods.
}
	\label{fig:rslts}
\vspace{-0.25in}
\end{figure}

MATLAB code to reproduce the results in this paper is at the first author's github repository \url{https://github.com/aabbas02/LowRankMatrixCompletion}. %\url{https://github.com/aabbas02}. 
For  AltGD \cite{yi2016fast}, we used the code provided by the authors of that work.
For ProjGD, AltMin (Fed./NotPrvt.) and AltMin(Fed./Prvt.), we wrote our own code. As explained in Sec. \ref{complexity}, the latter used GD to solve the LS problem for updating $\U$. We set the number of GD iterations for solving each LS problem to 10 and the step size to $\eta = p/\| \Y \|^2$. AltGDmin is implemented with two choices of the step size $\eta = c p/\| \Y \|^2$, $c = \{0.75,1\}$. This approximates the step size choice suggested by Theorem \ref{thrm} since $\E[\|\Y\|^2] = p \sigmax^2$.
We plot averaged subspace distance at the iteration $t$ against the average time taken until iteration $t$, with the averages being computed over 100 Monte Carlo runs. The averaging is over the observed entries which are generated uniformly at random.
The matrix $\Xstar = \Ustar \Bstar$ was generated once: we let $\Ustar$  be an orthonormalized $n \times r$ random Gaussian matrix and $\Bstar$ an $r \times q$ random Gaussian matrix.%
%
%
%The left-singular vectors $\U^*$ are generated by orhtonormalizing $\tilde \U$, where $\tilde \U$ is Gaussian i.i.d.  %The entries of matrix $\tilde\X  \in \mathbb{R}^{n \times q}$  are sampled i.i.d. from the normal distribution. Rank-$r$  matrix $\X^*$ is generated by truncating the $r$ singular vectors and singular values of $\tilde \X$. The resulting matrix has incoherence $\mu(\X^*) \simeq 1$.
%The step size for AltMin(Prvt.) was set equal to $\eta = p/\| \Y \|^2$. This choice of $\eta$ is based on an estimated upper bound of the initial operator norm $\| \mathbb{E}_{\Omega}[\nabla_\U f(\U,\B^{(0)})] \|$ \cite{allrtnPpr}. For AltGDMin, given Theorem \ref{thrm},  we estimate $\| \Y \| \simeq p \sigmax$ and set $\eta = cp/\| \Y \|^2$, $c = \{0.75,1\}$. While we may set $c < 1$ without changing the sample/iteration complexity, $c=0.75$ ensures that $\eta$ is small enough for Lemma \ref{lem:rowIncoh} to hold.

%Figure \ref{fig:rslts}  plots the subspace distance $\SE(\U^{(t)},\U^*)$ against time/seconds, averaged over 100 runs.

{\em The results show that the proposed method AltGDMin is the fastest, converging to $\Ustar$ in approximately 4 seconds, compared to second fastest AltMin(Fed. NotPrvt.) which takes nearly 8 seconds.}
%
%AltGDMin has a low run-time because it solves the $\B$-update least-squares (LS) problems locally, and in parallel, at the nodes. The up-stream communication complexity, $nr$, is also low because the nodes sum the column-wise gradients $\sum_k \nabla_{\U} f(\U,\b_k)$, where the summation is over the subset of columns $\b_k$ at the node, before transmitting to the center. %Consequently, the maximum upstream communication cost per-node is $nr$, compared to $\sum_{k} \lvert \Omega_k \rvert r$ if the gradients were transmitted without being summed.
%
%Next, we discuss the details of our federated simulation and also interpret the performance of other algorithms.
For both AltMin (Fed./NotPrvt) and AltGDMin, we used the `parfor' loop in MATLAB to distribute the $\B$ least-squares updates across 10 workers. AltMin (Fed./NotPrvt.) is not private because the nodes communicate the updated $\b_k^{(t+1)}$ to the center; it is slower than AltGDMin because the $n$ $\U$-update LS problems are solved sequentially at the center with complexity $\lvert \Omega \rvert r^2$, compared to the $nr^2$ complexity of computing the QR decomposition for AltGDMin.  For AltMin(Fed./Prvt.), the $\U$-update LS problems are solved by gradient descent at the nodes, as explained in Sec. \ref{sec:bnchmrks}.  While private, the GD version of AltMin is slow because of the communication overhead of transmitting the gradients several times in each iteration. AltMin (Cntrl.) is slow because both $\U$,$\B$ LS  problems are solved sequentially by the closed form solution at the center. We did not federate the implementations of ProjGD and AltGD. The reason is in case of ProjGD all the computation needs to be done at the center.
%has zero computational complexity per node (see Table \ref{tbl:1}) as the SVD computation is done at the center.
For AltGD, we computed the gradient by a matrix-matrix product at the center, which is faster than a matrix-vector product computation at the node and subsequent upstream transmission to the center. Therefore, for both algorithms, the federated implementations would have higher run-times because of the additional communication cost at each iteration.

More experiments (phase transition plots to evaluate sample complexity) are in Appendix \ref{long_sims} in longer version \cite{lrmc_altgdmin_arxiv}.%

%\begin{algorithm}
%	\caption{AltGDMin-Federated}
%	\begin{algorithmic}[1]
%		\label{algorithmFed}
%		\REQUIRE partial observations $\Y$,  rank $r$,  step size $\eta$, and number of iterations $T_{\text{init}}$, $T$
%		\STATE{Partition $\Y$ into $2T+1$ subsets $\Y_{\Omega^{(0)}}, \cdots, \Y_{\Omega^{(2T)}}$}
%		\STATE{//\textit{Compute Initialization $\U^{(0)}$ by Power Method}}
%		\STATE{\underline {Center}:  Initialize random $\U \in \mathbb{R}^{n \times r}$; transmit to $\gamma$ nodes}
%		\FOR {$t \in 1 \cdots T_{\text{init}}$}
%		\State{\underline {Nodes}: \text{ $\M_k  \gets \sum_{k \in \mathcal{S}_l}\y_{\Omega_k^{(0)}} \y_{\Omega_k^{(0)}}^\intercal \U \, \forall \, l \in [\gamma] $} }		
%		\State{\underline {Center}: $\U \gets \mathrm{QR}(\M)$}
%		\ENDFOR
%		\State{//\textit{AltGDMin Iterations}}
%		\FOR {$t \in 1 \cdots T$} %\vspace{0.08em}}
%			\State{\underline{Nodes}: $\b_k^{(t)} \gets (\U_{k}^{(t-1)})^{\dagger} \y_{\Omega_{k}^{(t)}} \, \forall \, k \in \mathcal S_l$, $l \in \gamma$}
%			\STATE{\underline{Center}: \text{$\tilde\U^{(t)} \gets \U^{(t-1)} - \eta(\U^{(t-1)}\B^{(t)} - \Y)_{\Omega^{(T + t)}} \B^{(t)}{}^\intercal$}}
%			\STATE{\underline{Center}: $\U^{(t)} \gets \mathrm{QR}(\tilde\U^{(t)})$}
%			%\STATE{$t \gets t + 1$}	
%	\ENDFOR
%	\STATE {\bfseries {Return} $\U, \B$}
%\end{algorithmic}
%\label{algo:alt-gd-min}
%\end{algorithm}



%The number of gradient descent (GD) iterations was set to 10.
%We observe that out of the two `private' algorithms, AltMin (Prvt.) and  AltGDMin, the proposed AltGDMin is significantly faster. For example, AltGDMin takes fewer than 10 seconds to converge to $\U^*$, compared to more than 20 seconds taken by AltMin (Prvt.).  AltGDMin also has a lower runtime than AltGD and ProjGD, two methods which are centralized and not private. We now describe the details of our distributed simulation setup. For both AltMin and AltGDMin, we used the `parfor' loop in MATLAB to distribute the $\U$ and $\B$ updates  across 4 workers.  The number of gradient descent iterations for AltMin (Prvt.) was set to 10. The least squares problems are solved exactly by the closed form solution for AltMin (Exact). The results show that, despite a small number  of GD iterations (10 iterations), the communication overhead of transmitting the individual gradient terms in equation \eqref{eq:gradSum} greatly increases the runtime of AltMin(Prvt.). We note that the run-time for AltGDMin includes the cost of the QR decomposition of $\U^{(t)}$ performed at the center whereas, for AltMin (Prvt.), the cost of adding up the individual gradient terms  from the nodes was neglected.



==> signalProcessingLetters/SPL_lrmc_phaseTransition.tex <==

\section{More Simulation Experiments}\label{long_sims}

\begin{figure}[!]
	\centering
	\begin{subfigure}[b]{0.35\textwidth}
		\centering
		\includegraphics[width=\textwidth]{phaseTransitionr5.pdf}
		\caption{}
		\label{fig:phaseTransitionr5}	
	\end{subfigure}
	\begin{subfigure}[b]{0.35\textwidth}
		\centering
		\includegraphics[width=\textwidth]{phaseTransitionr10.pdf}
		\label{fig:phaseTransitionr10}	
	\end{subfigure}
	\caption{Sample complexity comparison of AltGDMin with that of benchmark methods using phase transition plots. We plot a Monte Carlo estimate of the probability of the recovery error being below $10^{-10}$ for different values of $p$ (the probability of any entry of $\Xstar$ being observed).}
	\label{fig:phaseTrsntn}
\end{figure}

AltGDMin is compared with benchmark methods based on  sample complexity, that is, the number of observed entries required for successful matrix completion. We plot a Monte Carlo estimate of the probability of the recovery error being below $10^{-10}$ for different values of $p$ (the probability of any entry of $\Xstar$ being observed). %Observe that all of AltGDmin, AltMin%The results show that AltGDMin has lower sample complexity than ProjGD and AltGD, and slightly higher sample complexity than that of AltMin. We emphasize, however, that AltGDMin is faster in a distributed setting that AltMin.

